Beyond Scalar Probes: Exploiting Vector-Valued Outputs in ReLU Networks For Signature Extraction

We revisit cryptanalytic extraction of ReLU networks from a geometric and algebraic perspective. Rather than restricting attention to a single output component, we study the full vector-valued behavior across adjacent linear regions. This leads to a rank-one characterization of Jacobian differences that recovers the usual row-signature information while also revealing complementary column-side information. Our experiments show how this additional structure can be used in ex- traction and improves numerical estimation under different numerical- precision regimes (float64, float32 and float16). We extend the analysis beyond the high-precision and output-rounding settings commonly con- sidered in the literature towards the low-precision settings encountered in many practical settings.

==> Intro.tex <==
\section{Problem}
In the case of expanding network, there is no attack that can recover the hidden weights of a DNN where the activation function is $\Relu(x) = \max\{0,x\}.$
In the following I will present a new idea that can recover some information regarding the last layer starting from the output instead of starting from the input as in the previous attack.

It is still a seminal idea but I think it could be an interesting starting point.
I will assume we have access to the soft output with infinite precision.


\section{Idea}

We denote by $\bm v^{(i)} \in \R^{d_i}$ the vector constituted by the output of the $i$-th layer of a network where $d_i$ is the number of neurons in layer $i$.
The input will be $\bm v^{(0)} \in \R^{d_0}$  and the output will be $\bm v^{(\ell)} \in \R^{d_{\ell}}.$
Each layer after the $0$-th can be obtained from the previous as 
$$
   \bm v^{(i)} = \Relu(\bm A^{(i)}\bm v^{(i-1)} + \bm b^{(i)}),
$$
where $\Relu$ is applied to each component, $\bm A^{(i)} \in \R^{d_i \times d_{i-1}}$ and $\bm b^{(i)} \in \R^{d_i}$.

The output of the DNN can be expressed in terms of the second to last layer as
$$
    \bm v^{(\ell)} = \Relu(\bm A^{(\ell)}\bm v^{(\ell-1)} + \bm b^{(\ell)}).
$$

Observe that, if $d_{\ell} > d_{\ell-1}$, the vector 
$$
\bm w^{(\ell)} = \bm A^{(\ell)}\bm v^{(\ell-1)} + \bm b^{(\ell)} \in \Colsp(A^{(\ell)}) + \Span{}{\bm b^{(\ell)}},
$$
that is the vector $\bm w^{(\ell)}$ belongs to a subspace of dimension $d_{\ell-1} + 1.$
We can also observe that $\bm v^{(\ell-1)} = \Relu(\bm w^{(\ell - 1)})$ will have a zero entry for each of the negative components of $\bm w^{(\ell -1)} = \bm A^{(\ell-1)}\bm v^{(\ell-2)} + \bm b^{(\ell-1)}.$
Suppose there are $t \leq d_{\ell -1}$ non-zero entries of $\bm v^{(\ell-1)},$ the vector $\bm w^{(\ell)}$ will be the linear combination of just $t$ columns of $A^{(\ell)}$ and the unknown vector $\bm b^{(\ell)}.$

There is a way to remove the vector $\bm b^{(\ell)}.$
Consider the input $\bm v^{(0)}$ and the same input perturbed by a small vector $\bm v'^{(0)} = \bm v^{(0)} + \bm \delta_0.$ 
As the DNN is locally linear, then for each layer $\bm v'^{(i)} = \bm v^{(i)} + \bm \delta_i$ where $\bm \delta_i$ is also small vector.
In particular we have 
$$
    \bm w'^{(\ell)} = \bm A^{(\ell)}\bm (v^{(\ell-1)} + \bm \delta_{\ell -1}) + \bm b^{(\ell)} = \bm w^{(\ell)} +  \bm A^{(\ell)} \bm \delta_{\ell -1},
$$
from which we have that $\bm w'^{(\ell)} - \bm w^{(\ell)} = A^{(\ell)} \bm \delta_{\ell -1}$
where $\bm A^{(\ell)} \bm \delta_{\ell -1}$ belongs to the subspace generated by the $t$ columns of $\bm A^{(\ell)}$ corresponding to the non-zeroes entries of $\bm v^{(\ell - 1)}.$
(Notice that $\bm \delta_{\ell -1}$ will have the same non-zero components of $\bm v^{(\ell -1)}$ as we assume that a small change of the input will cause no transition from active to inactive in the neurons)

Starting from a vector $\bm v_1^{(0)}$ and slightly perturbing it in different directions we can generate different vectors belonging to the same subspace of $t_1 \leq d_{l-1}$ columns. 
After $t_1$ (or some more) of these perturbations we will recover a space $\calA_1$ of dimension $t_1$.
Taking a totally different input $\bm v_2^{(0)}$, it is likely that we will get a different configuration of active and inactive neurons in the layer $\ell -1.$
This means that we will get a different subspace $\calA_2$ of dimension $t_2$ generated by the columns of $\bm A^{(\ell)}$ corresponding to the active neurons in that layer.

Continuing in this way, we will have several subspaces $\calA_1, \ldots, \calA_n$.
Intersecting several of those we will get smaller and smaller subspaces (possibly zero).
We are interested in finding all the possible subspaces of dimension $1$ as those correspond to a single column of $\bm A^{(\ell)}$ up to a scalar.

\color{red}
Suppose the number of non-zero entries of $\bm v_1^{(\ell -1)}$ is $t_1.$
From what we just described, by small perturbations of $\delta_i$ on the input vector $\bm v_1^{(0)}$ we can collect some more then $t_1 < d_{\ell-1}$ outputs and generate the space of the columns of $\bm A^{(\ell)}$ corresponding to the non-zero entries of $v_1^{(\ell -1)}$.
The main issue is the following.
Suppose the first layer has $d_0 < t_1$ elements, or that any layer in between has $d_j < t_1$ elements and call $d_{\min} = \min \{d_0, \ldots, d_{\ell-2} \}.$
The vectors $\bm \delta_i^{(\ell -1)}$ all belong to a subspace of dimension at most $d_{\min} < t_1,$
therefore $\hat{\calA}_j = \Span{\R}{\bm A^{(\ell)} \bm \delta_i^{(\ell-1)} \mid i \in \{1, \ldots, t_1\}}$ will be at best a space of dimension $d_{\min}$ which is contained in the space generated by the $t_1$ columns of $\bm A^{(\ell)}$ corresponding to the non-zero entries of $\bm v_i^{(\ell -1)}$ (under the hypothesis that we stay in the same linear cell the non-zero entries of $\bm \delta_i^{(\ell -1)}$ are the same as the one of $v_i^{(\ell -1)}$).

At the moment, we do not know how to overcome this problem or use this fact.
Possibly this makes all this work a bit useless or maybe it could shade some light on unexplored territory.
In particular, if $d_{\min} < d_{\ell}$ then it means all the layers following the one where $d_i = d_{\min}$ have some redundancy.
In the sense that the linear operation described by $\bm A^{(t)}$ for $t >i+1$ is not really an operation from $\R^{d_{t-1}}$ to $\R^{d_{t}}$ as its domain will be limited to a subspace of $\R^{d_{t-1}}$ of dimension at most $d_{\min}.$
\color{black}

\section{Issues}
In the case of a (strongly) contractive model it could easily happen that all $\calA_i$ correspond to the whole space $\R^{d_\ell}$ making the above idea useless. \todo{would be interesting if we can express a bound here}
To give a bound we need some estimation of how many neurons on average are active or inactive in layer $\ell$ and $\ell - 1$.
A first heuristic would be a Bernoulli with probability $0.5$ for both of them and considering each node independent.
But I do not really think it is a good heuristic, there are clearly dependencies, especially if we assume the net was trained. 
For a random initialization it could be a roughly accurate model as I have no reason to believe positive values are more common than negative values.

\subsection{The main issues}
Here we assume to have access to $\bm w^{(\ell)}$ but the reality is that we have access only to $\bm v^{(\ell)},$ that is we cannot see the negative components of $\bm w^{(\ell)}$.
My intuition is that we can overcome this problem.

If the number of non-negative entries of $\bm v^{(\ell)}$ is $u>t,$ for $t < d_{\ell -1}$ the number of active neurons in the previous layer, we can find $\calA'$ of dimension $t$ a subspace of columns of $\bm A^{(\ell)}$ restricted to the support of $\bm v^{(\ell)}.$ (i.e. a subspace of dimension $t$ of $\R^u$ where $u$ is the size of the support of $\bm v^{(\ell)}$)

Collecting $\calA_i$ with similar supports and patiently gluing them together I think it is possible to slowly recover all the columns.\todo{would be nice if we can build a small example to show this}


Another problem is that we recover the columns up to some constant factor.
Without loss o generality, suppose we scale the first column by a positive factor $\lambda > 0,$ if we scale by $1/\lambda$ the first row of the preceding layer and the first component of the previous bias we will get a DNN functionally identical.
That is basically the same argument used in the papers we have seen, as in those papers we still have a problem of determining the sign.


\subsection{What about $\bm b^{(\ell)}$?}
In the process described so far, we did not address the problem of finding $\bm b^{(\ell)}.$
For simplicity suppose we have access to $\bm w^{(\ell)}$, or equivalently that we collect many outputs where $\bm v^{(\ell)}$ has full support.

Consider the spaces $\hat{\calA_i}$ generated by $\bm w_i, \bm w_i', \bm w_i'' \ldots$ instead of the spaces $\calA_i$ generated by $w_i-  w_i', w_i-  w_i'', \ldots$ of the other section.

Each $\hat{\calA_i}$ contains $\Span{\R}{\bm b^{(\ell)}}$, intersecting enough of them, we will remain only with the space $\Span{\R}{\bm b^{(\ell)}}.$
Again this is like finding $\bm b^{(\ell)}$ up to a constant multiplicative factor. We need to find a way to determine this factor. 

Let $\bm b \in \Span{\R}{\bm b^{(\ell)}},$ we want to find the correct factor $\lambda$ such that $\lambda \bm b = \bm b^{(\ell)}.$
Solving the system
$$
\begin{pmatrix}
    \bm A^{(\ell)} \mid \bm b 
\end{pmatrix}
\begin{pmatrix}
    \bm v^{(\ell-1)}\\
    \lambda
\end{pmatrix}
=
\bm w^{(\ell)}
$$
we will find the correct value of $\lambda.$

Observe that the components of $\bm v^{(\ell)}$ must be positive, if the solution we find has negative component in position $i$ it means we have to flip the sign of the $i$-th column of $A^{(\ell)}.$
To be honest this last step seems a bit too good to be true.

\todo{but the explanation sounds plausible}

\todo{maybe we could try to build a small example of DNN and try to do the process and see what happens. Something small enough that we can even work pen and paper method?}

==> MatchingAndGlue.tex <==
\section{Collect, match and glue}
The spaces $\calA_i$ we collect are the results of the combination of some columns of $\bm A$ to which we remove some rows.
The columns selected in $\calA_i$ correspond to the components of $\bm w_i^{(\ell -1)}$ that are $>0$ and the non-zero coordinates of $\calA_i$ corresponds to the positive coordinates of $\bm w_i^{(\ell)}.$
Locally, we can model the two component-wise ReLU as two diagonal matrices $R_i^{(\ell)}, R_i^{(\ell)}$ with $1$ on the main diagonal corresponding to the positive coordinates of $\bm w_i^{(\ell-1)}$ and $\bm w_i^{(\ell)}$ and $0$ on all the other entries.
Notice that, while these two matrices depend non-linearly on the input vector $\bm v_i^{(0)}$, locally they are constant and linear.
We hope to clarify with the following example:
Let,
$$
    \bm A^{(\ell)} = \begin{bmatrix}
  1.6 & -1.9 &  0.5 & -1.5 &  1.3 \\
 -1.0 &  0.7 & -0.3 & -1.8 & -0.3 \\
  1.4 & -1.4 & -1.3 &  1.9 &  0.6 \\
 -1.8 & -1.7 & -0.7 &  1.1 &  1.3 \\
 -0.4 & -0.7 &  1.8 &  1.8 &  1.3
\end{bmatrix}
$$
and let
$$
\bm w_i^{(\ell -1)} = (-1.5, 1.1, -1.5, 1.8, -2.0)^\intercal.
$$
The ReLU will act on $\bm w_i^{(\ell -1)}$ through the matrix 
$$
    R_i^{(\ell-1)} = \begin{bmatrix}
0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 0
\end{bmatrix}
$$
setting to zero its negative components.
This leads to
$$
\begin{bmatrix}
  1.6 & -1.9 &  0.5 & -1.5 &  1.3 \\
 -1.0 &  0.7 & -0.3 & -1.8 & -0.3 \\
  1.4 & -1.4 & -1.3 &  1.9 &  0.6 \\
 -1.8 & -1.7 & -0.7 &  1.1 &  1.3 \\
 -0.4 & -0.7 &  1.8 &  1.8 &  1.3
 \end{bmatrix}
 \begin{bmatrix}
0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 0
\end{bmatrix}
\begin{bmatrix}
-1.5 \\ 1.1 \\ -1.5 \\ 1.8 \\ -2.0
\end{bmatrix}
=
\begin{bmatrix}
-4.79 \\ -2.47 \\ 1.88 \\ 0.11 \\ 2.47
\end{bmatrix}.
$$
Finally we will apply another ReLU in the form of a matrix $\bm R_i^{(\ell)}$ to the obtained vector obtaining
$$
    \bm v_i^{(\ell)} = (0 , 0 , 1.88 , 0.11 ,2.47). 
$$

This is the same as
\begin{align}  
&\begin{bmatrix}
0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 \\
0 & 0 & 1 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 1
\end{bmatrix}
 \begin{bmatrix}
  1.6 & -1.9 &  0.5 & -1.5 &  1.3 \\
 -1.0 &  0.7 & -0.3 & -1.8 & -0.3 \\
  1.4 & -1.4 & -1.3 &  1.9 &  0.6 \\
 -1.8 & -1.7 & -0.7 &  1.1 &  1.3 \\
 -0.4 & -0.7 &  1.8 &  1.8 &  1.3
 \end{bmatrix}
 \begin{bmatrix}
0 & 0 & 0 & 0 & 0 \\
0 & 1 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 1 & 0 \\
0 & 0 & 0 & 0 & 0
\end{bmatrix}
\begin{bmatrix}
-1.5 \\ 1.1 \\ -1.5 \\ 1.8 \\ -2.0
\end{bmatrix}
\\
& = 
\begin{bmatrix}
 0 &  0   & 0 &  0   & 0 \\
 0 &  0   & 0 &  0   & 0 \\
 0 & -1.4 & 0 &  1.9 & 0 \\
 0 & -1.7 & 0 &  1.1 & 0 \\
 0 & -0.7 & 0 &  1.8 & 0
 \end{bmatrix}
\begin{bmatrix}
-1.5 \\ 1.1 \\ -1.5 \\ 1.8 \\ -2.0
\end{bmatrix}
=
\begin{bmatrix}
0 \\ 0 \\ 1.88 \\ 0.11 \\ 2.47
\end{bmatrix}.
\end{align}

The vector space we can recover with our technique is the one given by the span of the two non-null columns after we set to $0$ the first two rows.
That is $\calA_i = \Span{\R}{(0,0,-1.4,-1.7,-0.7)^\intercal,(0,0,1.9,1.1,1.8)^\intercal}$.


%To each subspace we can assign a support given by the coordinates that are not constantly $0$. 
%The support is a subset of the interval $[n] := \{ 1,\ldots,n \},$ in our example it would be the set $S(\calA_i) = \{3,4,5\} \subseteq [5].$
%Similarly, the support of a vector is given by the set of the coordinates where it is not null.
%To each support $S$ we can assign a standard vector $\bm \chi_S$ of length $n$ that is $1$ for each coordinate in $S$ and $0$ otherwise.
%Notice that $\bm R_i^{(\ell)} = \Diag(\bm \chi_{S(v_i^{(\ell)})})$

The support is a subset of the interval $[n] := \{ 1,\ldots,n \},$ in our example it would be the set $S_i = \{3,4,5\} \subseteq [5].$
Suppose we have two subspaces $\calA_1,\calA_2$ with the same support, their intersection will correspond to the space generated by the columns of $\bm R_1^{(\ell)} \bm A  \bm R_1^{(\ell -1)}$ and $\bm R_2^{(\ell)} \bm A  \bm R_2^{(\ell -1)}.$
Notice that, with probability $1$, the two subspaces will have the same support if and only if $\bm R_1^{(\ell)}= \bm R_2^{(\ell)}.$
Also the intersection will be given by the columns of $\bm R_1^{(\ell)} \bm A \bm R_1^{(\ell -1)} \bm R_2^{(\ell -1)}.$
Where $\bm R_1^{(\ell -1)} \bm R_2^{(\ell -1)}$ is the $\Relu$ matrix of the intersection between the supports of $\bm v_1^{(\ell-1)}$ and $\bm v_2^{(\ell-1)}.$

If $\calA_1 \cap \calA_2$ has dimension $1$ this corresponds to a column of $\bm R_1^{(\ell)} \bm A$ up to some scalar multiplication.
We will refer to a generator of this space as a partial column of $\bm A$.

In order to get all the columns of $\bm A^{(\ell)}$ up to some scalar we need to solve the following two problems.
A first problem is that spaces with exactly the same support are rare, so we need an alternative way to obtain partial columns.
A second problem is how to get a complete a column from several partial columns.
We will address the two questions in the following two paragraphs.

\paragraph{Collect partial columns (Expand and cutting)}
A first problem is that two subspaces $\calA_1, \calA_2$ could have two different supports.
Our algorithm collects all the partial subspaces $\calA_i$ together with their support $S_i \subseteq [n]$ forming the pair $(\calA_i, S_i)$
We can sort this list of pairs by putting first the pairs with a larger support.
As we cannot expect to have many subspaces with exactly the same support, we can do the following.
We pick the first pair $(\calA_1,S_1)$ and consider all the pairs such that $S_i \subseteq S_1.$
If $S_i \subsetneq S_1$, as it is generally the case, we can extend $\calA_i$ with the space $\Span{\R}{e_{i_1}, \ldots, \bm e_{i_t}}$ where $\bm e_i$ are element of the standard basis and $I_{1,i} = \{i_1, \ldots, i_t\} = S_1 \setminus S_i.$
The new space $\calA_i' = \calA_i + \Span{\R}{e_{i_1}, \ldots, \bm e_{i_t}}$ will have the same support of $\calA_1.$
Its dimension will be $\dim(\calA_i) + t$ and it is generated by some partial columns of $\bm A^{(i)}$ plus some element of the standard basis.

Without loss of generality suppose the support of $\calA_i$ is $[k] = \{1,\ldots, k\}$ and the support of $\calA_i'$ is equal to $[k+t].$
Suppose that $\calA_i$ contains the first partial column of $\bm A^{(\ell)}$. 
That is, the first column of $\bm A^{(\ell)}$ where we substitute with $0$ all the components after the first $k.$
In $\calA_i'$ among many other vectors, there will also be the partial column up to the $k+t$ component.

Thanks to this trick all the expanded vector spaces will contain a larger version of their partial columns matching all with the same support $S_1.$

If we intersect $\calA_1$ with $\calA_i$ and the two have some columns in common we will obtain a space that is given by the span of the common columns.
We are interested in the cases when there is only one column in common as this will directly give us a partial column.
\\

\textbf{Some caveats}

If we intersect two expanded set we could easily get spaces generated by the same vectors $\bm e_i$ we used to expand.
We are implicitly assuming that $\calA_1$, as is the only space we do not expand, do not contain any vector from the standard basis. (this is a fair assumption as this has probability $0$ to happen)
This means we should always include the space $\calA_1$ when we do the intersections with the other expanded spaces whose original support was contained in $S_1.$
\\

The space $\calA_1$ will in general contain only some columns and will also be partial, so we need to repeat this procedure for some different partial spaces $\calA_i,S_i$ in the partially ordered list until we collect enough partial columns.
\\

Another risk when expanding is to include things that should not be included ``ghost partial columns".
Suppose the support of the space $\calA_1$ is of size $d_{\ell} - s$ and let be $\calA_i$ the space with which we want to intersect.
In general we will have $\dim(A_i') = \dim(A_i) + t$  where $t = |S_1 \setminus S_i|$ and
$$
    d_{\ell} - s \geq \dim(\calA_1 + \calA_i') = \dim(\calA_1) + \dim(\calA_i') - \dim(\calA_1 \cap \calA_i'),
$$
from which we get
$$
    \dim(\calA_1 \cap \calA_i') \geq \dim(\calA_1) + \dim(\calA_i) + t - d_{\ell} + s.
$$
Notice that this means that for some values of $s$ and $t$ there could be an intersection even if $\calA_i$ and $\calA_1$ have no columns in common.
In practice we should avoid to expand spaces that have a too small support compared to the target or verify that on the right side of this inequality we have something $\leq 0.$ 
In this way we should be safe from meeting some ghost space.
(That was actually the source of some errors in my first naive implementation)


\paragraph{From partial to full columns (Patiently gluing)}
After the procedure described in the previous paragraph, we end up with many partial columns.
The problem is how to get a full column starting from some partial columns.

A first step is to group partial columns that comes from the same column.

Suppose we have two partial columns such that their support is intersecting in more than two entries.
To check if these two columns belong are coming from the same column we have to find a scalar such that, on their intersection they are equal.
Let $\bm v, \bm w$ be these two columns and suppose $S_v \cap S_w = \{ i,j \}.$
If we consider the vectors $\bm v' = v_{i}^{-1}  \bm v$ and $\bm w' = w_{i}^{-1} \bm w$ they will be both $1$ in their $i$-th component and, if they come from the same column, $v_j' = w_j'.$
This will be already enough to state that $\bm v,\bm w$ come from the same column with probability $1.$
If we do not trust that their are equal only over one component (besides the component equal to $1$ by construction) we can test for all the components that are in the support intersection.

With this same idea we can also gluing together two partial columns relative to the same column of $A^{(\ell)}$.

Let again $\bm v,\bm w$ be two partial columns relative to the same column. 
After we ``normalize" them in the first component of their support intersection, we will notice that they are the same over all the intersection.
The original column will also be the same on this intersection once we set to $1$ that component, moreover all the other components that appear in the two vectors will be the same as the ``normalized" column.
This means that, starting from two partial columns of support $S_v, S_w$ we get a partial columns of support $S_v \cap S_w,$ repeating this gluing process we can end up recovering the whole column if $S_v \cap S_w = [n].$
\\

\textbf{Example}\\
We illustrate better this idea with an example.
Let $\bm v = (1,2,3,0)^\intercal, \bm w = (0,4,6,4),$ be two partial columns. 
Their supports are $S_v = \{1,2,3\}$ and $S_w= \{2,3,4\}$ so $S_v \cap S_w = {2,3}.$
We set them both to $1$ in the second component by multiplying by $1/v_2$ and $1/w_2$ respectively, obtaining
$$
\bm v' = \begin{pmatrix}
    \frac{1}{2} \\ 1 \\ \frac{3}{2} \\0
\end{pmatrix}, \quad
\bm w' = \begin{pmatrix}
    0 \\ 1 \\ \frac{3}{2} \\ 1
\end{pmatrix}.
$$
We verify that their $3$-rd component is the same which means we can glue them together obtaining 
$$
\mathrm{Glue}(\bm v, \bm w) = \begin{pmatrix}
    \frac{1}{2} \\ 1 \\ \frac{3}{2} \\1
\end{pmatrix}.
$$

==> Preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Notation}
We denote by $\R$ the set of real numbers. 
The vector space of $n$-tuples of real numbers is denoted by $\R^n$.
Vectors are written in bold lowercase letters, such as $\bm v \in \R^{n}$, and are interpreted as column vectors unless otherwise stated. 
Similarly, the transpose $\bm v^\intercal$ will be interpreted as a row vector.
For a vector $\bm v$, its $i$-th component is denoted by $v_i$.


Matrices with real entries $m$ rows and $n$ columns are elements of $\mathbb{R}^{m \times n}$, and are denoted by bold uppercase letters, such as $\bm M$.
The $i$-th row of $\bm M$ will be indicated by the row vector $\bm m_{i,*}^\intercal$ and the $j$-th column of the same matrix will be indicated by $\bm m_{*,j}.$
The transpose of a matrix $\bm M \in \R^{m \times n}$ will be indicated by $\bm M^{\intercal} \in \R^{n \times m}$.
Given two functions $f(x),g(x)$, we will indicate their composition as $f \circ g(x)= f(g(x))$ 

\subsection{Model Extraction}

Model extraction attacks are a cybersecurity problem that aims to compromise the confidentiality of the internal parameters of a machine learning model that is accessible as a black box~\cite{tramer2016stealing}. 
Model extraction attacks are generally divided into two main categories: task accuracy extraction~\cite{tramer2016stealing} and fidelity extraction~\cite{jagielski2020high}.
By task accuracy extraction, we mean that the stolen model will perform similarly to the original model on the training database and on data coming from the same distribution as the training database.
By fidelity extraction, we mean that the two models perform similarly over any possible input.
%Our work focuses on the second category, which aims to copy the model's predictions with the highest accuracy. 

The theoretical foundation of this field was laid by Fefferman's~\cite{fefferman1994reconstructing} 1994 study, which demonstrated that the weights of a network's output information can be uniquely determined. This fundamental research was further developed by Lowd and Meek~\cite{lowd2005adversarial} in 2005. 

\subsection{Deep Neural Networks}

A deep neural network can be described as a composition between affine functions over vectors with real coordinates and activation functions in the following way.

\begin{definition}[$\ell$-layer deep neural network]
\label{def:DNN}
    Let $n_0, \ldots, n_\ell$ be $\ell$ positive integers and let $A^{(1)}(\bm x),\ldots ,A^{(\ell)} (\bm x)$ be affine functions of the form
    \begin{equation}\label{eq:affine_function}
        A^{(k)}(\bm x) = \bm W^{(k)} \bm x + \bm b^{(k)},
    \end{equation}
    
    where $\bm W^{(k)} \in \R^{n_{k} \times n_{k-1}}$ is known as the \textbf{weight matrix} and $\bm b^{(k)} \in \R^{n_k}$ is known as the \textbf{bias vector} where $n_0$ is the length of the input, $n_\ell$ is the length of the output.\todo{we need to explain from where we come to these dimensions and what are rows and columns}
    
    An \textbf{$\ell$-layer deep neural network} is a function $F: \R^{n_0} \rightarrow \R^{n_{\ell}}$ (there are then in fact $\ell +1$ layers but, by convention, we do not count the input layer) of the form
    \begin{equation}
        \label{eq:DNN}
        F(\bm x) = A^{(\ell)} \circ \bm \sigma \circ \cdots \circ A^{(2)} \circ \bm \sigma \circ A^{(1)}(\bm x)
    \end{equation}
    where $\bm \sigma: \R^{n_k} \rightarrow \R^{n_k}$ denotes the component-wise application of the \textbf{activation function} $\sigma: \R \rightarrow \R$.

\end{definition} 


While in the above definition $\sigma$ is generic, from now on, we will restrict to the case where $\sigma$ is the $\Relu$ function.
$\Relu$ function is defined as $\sigma(x) = \max\{0,x\}$.
\color{blue}
A natural representation of an $\ell$-layer neural network is a directed graph of $N =  n_0+ \cdots + n_{\ell}$ nodes (see Figure \ref{fig:NN}). 
These nodes are arranged in subsets $L_0, \ldots, L_{\ell}$ called layers containing $n_0,\ldots,n_\ell$ nodes respectively.
Nodes are labeled as $\eta_i^{(k)}$ to indicate the $i$-th element of the $L_k$ layer.
Edges are directed and possible only between nodes in consecutive layers.
That is the edge $(\eta_j^{(k)}, \eta_i^{(t)})$  can exist only if $t = k+1$

A weight $w_{i,j}^{(k)} \in \R$ is associated to each edge $(\eta_j^{(k-1)},\eta_i^{(k)}).$
A bias $b_i^{(k)} \in \R$ is associated to each node $\eta_i^{(k)}$ with the exception of the first layer $ k=0.$
\color{black}

\begin{figure}
\centering
\begin{tikzpicture}[
    x=2.4cm, y=1.2cm,
    >=Latex,
    neuron/.style={circle, draw, minimum size=9mm, inner sep=0pt},
    every path/.style={->, thick}
]

% Number of nodes in each layer
\def\nzero{3}   % input layer L_0
\def\none{4}    % hidden layer L_1
\def\ntwo{3}    % hidden layer L_2


%--------------------------------
% Layer 0 (input)
%--------------------------------
\foreach \i in {1,...,\nzero} {
    \node[neuron] (L0-\i) at (0, {(\nzero+1)/2 - \i}) {$\eta_{\i}^{(0)}$};
}

%--------------------------------
% Layer 1
%--------------------------------
\foreach \i in {1,...,\none} {
    \node[neuron] (L1-\i) at (1.8, {(\none+1)/2 - \i}) {$\eta_{\i}^{(1)}$};
}

%--------------------------------
% Layer 2
%--------------------------------
\foreach \i in {1,...,\ntwo} {
    \node[neuron] (L2-\i) at (3.6, {(\ntwo+1)/2 - \i}) {$\eta_{\i}^{(2)}$};
}



%--------------------------------
% Edges between consecutive layers
%--------------------------------
\foreach \j in {1,...,\nzero} {
    \foreach \i in {1,...,\none} {
        \draw (L0-\j) -- (L1-\i);
    }
}

\foreach \j in {1,...,\none} {
    \foreach \i in {1,...,\ntwo} {
        \draw (L1-\j) -- (L2-\i);
    }
}


%--------------------------------
% Example labels for some weights
%--------------------------------
%\node[fill=white, inner sep=1pt] at ($(L0-1)!0.5!(L1-2)$) {$w_{2,1}^{(1)}$};
%\node[fill=white, inner sep=1pt] at ($(L1-3)!0.5!(L2-1)$) {$w_{1,3}^{(2)}$};
%\node[fill=white, inner sep=1pt] at ($(L2-2)!0.5!(L3-1)$) {$w_{1,2}^{(3)}$};

%--------------------------------
% Optional annotation for activation

\end{tikzpicture}
\caption{Directed graph representation of a simple neural network}
\label{fig:NN}
\end{figure}
\todo{maybe a nice graph depicting this?}

Each node can take a value in $\R$.
The first layer is initialized by the entries of the input $\bm x^{(0)}\in \R^{n_0}$.
For $k>0$, the node $\eta_i^{(k)}$ will take the value of the associated function $\eta_i^{(k)}(\bm x): \R^{n_{k-1}} \rightarrow \R$ defined as\footnote{Compare the argument of the function $\sigma$ in the definition above with
Eq.~\eqref{eq:affine_function} to see the connection between the weight matrix $\bm W^{(k)}$, the bias $\bm b^{(k)}$ vector and this formula.}
\begin{equation}
\label{eq:neuron}
    \eta_i^{(k)}(\bm x) = \sigma \left( \sum_{j=1}^{n_{k-1}} w_{i,j} ^{(k)} x_j  + b_i \right)
\end{equation}

The output of $\eta_i^{(k)}(\bm x)$ will be denoted in short by $x_i^{(k)}$, the ouput of all the neurons in the same layer $L_k$ form a vector 
\[
    \bm x^{(k)} = (\eta_1^{(k)}(\bm x^{(k-1)}), \ldots,  \eta_{n_k}^{(k)}(\bm x^{(k-1)})) = (x_1^{(k)}, \ldots, x_{n_k}^{(k)}).
\]

\begin{definition}\label{def:neuron}
    The functions $\eta_i^{(k)}: \R^{n_{k-1}} \rightarrow \R$ defined in (\ref{eq:neuron})  
are called \textbf{neurons}.
The \textbf{neuron} $\eta_i^{(k)}$ is associated with a node in the $k$-th layer; we use the same symbol to denote both the function and the node to which it is associated. 
The input coordinates of each function on the $k$-th layer will be the output of neurons in the previous layer. The input vector common to all the neurons in the $k$-th layer is denoted by $\bm x^{(k-1)}$.  
\end{definition}
\todo{difficult to read} 


\begin{figure}[H]
\centering
\begin{tikzpicture}[
    x=2cm, y=1.5cm,
    >=stealth,
    neuron/.style={circle, draw, minimum size=10mm, inner sep=0pt},
    smallneuron/.style={circle, draw, minimum size=8mm, inner sep=0pt}
]

% Previous layer neurons
\node[smallneuron] (x1) at (0, 1) {$\eta_1^{(k-1)}$};
\node[smallneuron] (x2) at (0, 0) {$\eta_2^{(k-1)}$};
\node[smallneuron] (x3) at (0,-1) {$\eta_3^{(k-1)}$};

% Main neuron
\node[neuron] (n) at (3,0) {$\eta_j^{(k)}$};

% Bias label
\node at (3.3,0.5) {$b_j^{(k)}$};

% Outgoing arrow
\draw[->, thick] (n) -- (5,0);

% Incoming arrows
\draw[->, thick] (x1) -- node[midway, above] {$w_{1,j}$} (n);
\draw[->, thick] (x2) -- node[midway, above] {$w_{2,j}$} (n);
\draw[->, thick] (x3) -- node[midway, above] {$w_{3,j}$} (n);

\end{tikzpicture}
\caption{Graphical representation of a neuron.}
\label{fig:neuron}
\end{figure}

The formula for the transition from layer $k-1$ to layer $k$ can be summarized as
\begin{equation}
\label{eq:update_gen}
    \bm x^{(k)} = \sigma \left( \bm W^{(k)} \bm x^{(k-1)} + \bm b^{(k)} \right ),
\end{equation}
where $\bm x^{(k-1)}$ and $ \bm x^{(k)}$ denote the output of the $(k-1)$-th and $k$-th layer, respectively, and, with an abuse of notation, we indicate by $\sigma$ the activation function $\sigma$ applied component-wise.



\color{blue}
Typically, in the last layer, the activation function is the max (in the case of hard label) and the $\mathrm{softmax}$ (in the case of soft label).
In the latter case, the output can be written as:
\begin{equation}
    \bm x^{(\ell)} = \mathrm{softmax}( \bm W^{(\ell)} \bm x^{(\ell-1)} + \bm b^{(\ell)}).
\end{equation}

For the rest of the paper, we will assume we have access to the raw output before the softmax:
\begin{equation}
    \label{eq:out_layer}
    \hat{\bm x}^{(\ell)} =  \bm W^{(\ell)} \bm x^{(\ell-1)} + \bm b^{(\ell)}.
\end{equation}
For ease of notation, we denote $\hat{\bm x}^{(\ell)}$ as $\bm x^{(\ell)}.$ 
\color{black}

When the activation function is $\Relu,$ neurons can be in different states according to their input.
\begin{definition}
    [critical point {\cite{carlini2020}}]
    Consider a neuron $\eta_i^{(k)}$ whose activation function $\sigma$ is $\Relu$.
    $$
        \eta_i^{(k)}(\bm x) = \Relu (\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)}). 
    $$
    The neuron is said to be in an \textbf{active state} if $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} > 0$. Next, it is said to be in an \textbf{inactive state} if $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} < 0$. Finally, it is said to be in a \textbf{critical state} if $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} = 0.$
    A point $\bm x$ such that $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} = 0$ is said to be a \textbf{critical point}.
The set of all the critical points constitutes a hyperplane named the \textbf{critical hyperplane}
$$
    \calH_{i}^{(k)} := \{\bm x \in \R^{n_{k-1}} \mid \bm w_i^{(k)\intercal} \bm x = -b_i^{(k)}\} .
$$
This hyperplane divides the space $\R^{n_{k-1}}$ between an \textbf{active area} corresponding to all the points such that $\bm w_i^{(k)\intercal} \bm x + b_i^{(k)} >0$ and an \textbf{inactive area} corresponding to the set of all points for which
$\bm w_i^{(k)\intercal} \bm x + b_i^{(k)} <0$.
\end{definition}
The critical hyperplane is parallel to the $(n_{k}-1)$-dimensional space $\bm w_i^{(k)\perp} := \{\bm x \in \R^{n_{k-1}} \mid w_i^{(k)\intercal} \bm x = 0 \}$. In particular, the vector $\bm w_i^{(k)}$ is orthogonal to the underlying space of the hyperplane $\calH_{i}^{(k)}.$
This observation was exploited in  \cite{shamir_carlini24} to recover the vectors $\bm w_i^{(k) \intercal}$ up to some scalar.
An equivalent way of extracting these vectors was first developed in \cite{carlini2020} through differential techniques.

\subsection{Invariant Transformation of Neural Network and Signature}

In Definition \ref{def:DNN}, we defined $F$ as a composition of affine functions $A^{(k)}(\bm x) = \bm W^{(k)} \bm x + \bm b^{(k)}$ interleaved by activation functions $\bm \sigma.$
Notice that, as $\bm \sigma$ acts component-wise, for any permutation $P_{n_k}$ of the positions (the coordinates) in $\R^{n_k},$ we have that $\bm \sigma(P_{n_k} \bm x) = P_{n_k}\bm \sigma(\bm x)$.
Then, the function $F$ is preserved under the transformation
$$
    F(\bm x) = A^{(\ell)} \circ \cdots \circ (A^{(k+1)} \circ P_{n_k}^{-1} )\circ \sigma^{(n_k)} \circ (P_{n_k} \circ A^{(k)})\circ  \cdots \circ A^{(1)}(\bm x).
$$
When the activation function is $\Relu$, there is another transformation of the affine functions that preserves $F$.
Notice that $\Relu(a x) = a \Relu(x)$ for any $a > 0.$
Multiplying by $a$ the output of a neuron $\eta_i^{(k)}$, is the same as multiplying by $a$ the $i$-th row of $\bm W^{(k)}$ and $b_i^{(k)}$.
If we also multiply by $a^{-1}$ the $i$-th column of $\bm W^{(k+1)}$, this will offset the previous operation, leading to the same output in the $(k+1)$-th layer.

\color{blue}
More in general, 
\[
\bm W^{(k+1)}\bm \sigma (\bm W^{(k)} \bm x + \bm b^{(k)})  + \bm b^{(k+1)} 
= \bm W^{(k+1)} \bm D^{-1} \bm \sigma (\bm D\bm W^{(k)} \bm x + \bm D\bm b^{(k)})  + \bm b^{(k+1)}
\]
were $\bm D$ is a diagonal matrix whose diagonal elements are all strictly positive, we can always construct an equivalent 
network where the elements in the first column of each $\bm W^{(i)}$ for $i < \ell$ are equal to $\pm 1$.

mention signatures \dots \todo{ermes: we define signatures right after in Definition \ref{def:signature}} in the following we will always assume that the element in the first column equals 1.

Suggestion 2: 
we could also declare that in each matrix the top rows are the linearly independent ones.
(if this helps the description or the recovery algorithm)
\color{red} ermes: Do not get what you mean, unless the system is designed to have linearly dependent rows it is extremely uncommon to have them by chance (measure zero event)
\color{black}
This leads to the following notion of neuron signature.
\begin{definition}[Signature]\label{def:signature}
Let $\eta_i^{(k)}(\bm x) = \sigma(\bm w_{i}^{(k) \intercal} \bm x  + b_i^{(k)})$ be a neuron on the $k$-th layer.
the \textbf{row-signature} \cite[Definition~4]{canales23} of $\eta_i^{(k)}$ is the row vector
$$
   (w_{i,1}^{(k)})^{-1} \bm w_{i}^{(k) \intercal} = \left (1,\frac{ w_{i,2}^{(k)}}{ w_{i,1}^{(k)}},\ldots, \frac{ w_{i,n_k}^{(k)}}{ w_{i,1}^{(k)}}\right ).
$$
That is the $i$-th row of $\bm W^{(k)}$ normalized on its first component.

In the same way, we can define a \textbf{column-signature} for the columns of $\bm W^{(k)}$ normalized on their first components.
\end{definition}

As neurons are invariant only to positive scalars, it is also important to determine the sign of the neuron.
Geometrically, a signature describes the critical hyperplane of a neuron, but it does not tell which of the two sides is active or inactive.
This information is contained in the sign, and it is fundamental to reconstruct a neural network functionally equivalent to $F$.



==> SecondOrderDerivative.tex <==



\section{Second order difference method}
In our work, we are trying to extend what was done in \cite{carlini2020} and continued in \cite{canales23}. We will give a brief description of this work and then describe our technique.
From now on, we will consider only neural networks whose activation functions $\sigma$ are given by the piecewise linear function $\Relu$  defined as $\Relu(x) = \max\{ 0, x\}.$

\begin{definition}[piecewise linear function]
A function $F: \R^n \rightarrow \R^m$ is said to be \textbf{piecewise linear} if there exists a finite collection $\calC =\{C_1, \ldots, C_t \},$ where $C_i$ are the sets of solutions to systems of linear inequalities such that $\bigcup_{i=1}^t C_i = \R^n $ and
$$
    F_{|C_i}(\bm x) = \bm W_i \bm x + \bm b_i,
$$ 
where $F_{|C_i}$ denotes the restriction of $F$ to the set $C_i$ and $\bm W_i \in \R^{m \times n}, \bm b_i \in \R^{m}.$
In other words, the restriction of $F$ to the sets $C_i$ is an affine function.
The sets $C_i$ are also known as \textbf{linear cells}.
\end{definition}
As anticipated, an example of piecewise linear function is given by the $\Relu$, indeed $\Relu_{|(-\infty, 0]}( x) = 0$ and $\Relu_{|[0,+\infty)}(x) = x$  are constant and linear respectively.
Moreover the union of the two intervals $(-\infty, 0], [0,+\infty)$ is equal to the whole domain $\R.$

The composition of affine functions and piecewise linear functions (in this case the $\Relu$) results in piecewise linear functions whose linear cells are delimited by portions of hyperplanes.

\begin{definition}
    [critical point {\cite{carlini2020}}]
    Consider a neuron $\eta_i^{(k)}$ whose activation function is $\sigma= \Relu$.
    $$
        \eta_i^{(k)}(\bm x) = \Relu (\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)}) 
    $$
    The neuron is said to be in an \textbf{active state} if $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} > 0$, it is said to be in an \textbf{inactive state} if $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} < 0$ and it is said to be in a \textbf{critical state} if
    $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} = 0.$
    A point $\bm x$ such that $\bm w_i^{(k)\intercal} \bm x + \bm b_i^{(k)} = 0$ is said to be a \textbf{critical point}.
The set of all the critical points, constitutes a hyperplane named the \textbf{critical hyperplane}
$$
    \calH_{i}^{(k)} := \{\bm x \in \R^{n_{k-1}} \mid \bm w_i^{(k)\intercal} \bm x = -b_i^{(k)}\} .
$$
This plane divides the input space between an \textbf{active area} corresponding to all the points such that $\bm w_i^{(k)\intercal} \bm x + b_i^{(k)} >0$ and an \textbf{inactive area} corresponding to the set of all points for which
$\bm w_i^{(k)\intercal} \bm x + b_i^{(k)} <0$. 
\end{definition}
The critical plane is parallel to the $(n_{k}-1)$-dimensional space $\bm w_i^{(k)\perp} := \{\bm x \in \R^{n_{k-1}} \mid w_i^{(k)\intercal} \bm x = 0 \},$
in particular, the vector $\bm w_i^{(k)}$ is orthogonal to the underlying space of the hyperplane $\calH_{i}^{(k)}.$

This observation was exploited in \cite{carlini2020},\cite{canales23}, \cite{shamir_carlini24} to recover the vectors $\bm w_i^{(k) \intercal}$ up to some scalar.
\color{blue}
In the more recent paper \cite{shamir_carlini24} the signature is indeed calculated collecting enough independent points on the hyperplane defining the relative neuron, in the older \cite{carlini2020} and \cite{canales23} the neuron recovering is presented as the solution of a system of equations.
The two methods are substantially equivalent and both suffer the same problem of not being able to find a signature if it is not possible to find enough linearly independent equations or sufficiently many independent points on the hyperplane.
This problem is more common in the case of an expansive neural network but, even in a non-expansive network, due to the $\Relu$ function, we can have a rank loss of the function at an intermediate layer and not being able to find sufficiently many independent equations.
In \cite{liu2025} this problem was overcome by combining linear equations coming from distinct portions of hyperplanes relative to the same neuron. 
The key observation is that this would give a one dimensional space if two or more of the equations are relative to the same neuron while it would give no solution if the equations were relative to distinct neurons.
We will describe the signature extraction process with more details in the next section.
\color{black}

Let $F$ be the function implemented by a neural network described by
$$
F(\bm x) = A^{(\ell)} \circ \sigma^{(n_{\ell -1})} \circ \cdots \circ A^{(2)} \circ \sigma^{(n_1)} \circ A^{(1)}(\bm x).
$$
Notice that, as $\sigma^{(k)}$ acts component-wise, for any permutation $P_{n_k}$ of $\R^{n_k},$ we have that $\sigma^{(k)}(P_{n_k} \bm x) = P_{n_k}\sigma^{(k)}(\bm x)$.
Then, the function $F$ is preserved under the transformation
$$
    F(\bm x) = A^{(\ell)} \circ \cdots \circ (A^{(k+1)} \circ P_{n_k}^{-1} )\circ \sigma^{(n_k)} \circ (P_{n_k} \circ A^{(k)})\circ  \cdots \circ A^{(1)}(\bm x).
$$
When the activation function is the $\Relu$, there is another transformation that preserves $F$.
Notice that $\Relu(a x) = a \Relu(x)$ for any $a > 0.$
This means that, multiplying by $a$ the output of a neuron $\eta_i^{(k)}$, is the same as multiplying by $a$ the $i$-th row of $\bm W^{(k)}$ and $b_i^{(k)}$.
Multiplying by $a^{-1}$ the $i$-th column of $W^{(k+1)}$ will offset the operation we did on the $k$-th layer, leading to the same output in the $(k+1)$-th layer.
This means that it is enough to recover all the rows or columns of each matrix up to a positive scalar without any particular order.
Because of the positive scalar invariant, it is natural to consider the neurons up to scalar, this leads to the following notion of a neuron signature.
\begin{definition}[Signature]
Let $\eta_i^{(k)}(\bm x) = \sigma(\bm w_{i}^{(k) \intercal} \bm x  + b_i^{(k)})$ be a neuron on the $k$-th layer.
the \textbf{row-signature} \cite[Definition~4]{canales23} of $\eta_i^{(k)}$ is the row vector
$$
   (w_{i,1}^{(k)})^{-1} \bm w_{i}^{(k) \intercal} = \left (1,\frac{ w_{i,2}^{(k)}}{ w_{i,1}^{(k)}},\ldots, \frac{ w_{i,n_k}^{(k)}}{ w_{i,1}^{(k)}}\right ).
$$
That is the $i$-th row of $\bm W^{(k)}$ normalized on its first component.

In the same way, we can define a \textbf{column-signature} for the columns of $\bm W^{(k)}$ normalized on their first components.
\end{definition}

The main tool used in \cite{carlini2020} and  the in the following works \cite{canales23}, \cite{shamir_carlini24}, is to recover the row-signatures of the various neurons from the vectors normal to the portions of hyperplanes delimiting the linear cells in the input space.
To find these hyperplanes two points $\bm x_1^{(0)}, \bm x_2^{(0)} \in \R^{n_0}$ are selected in the input space.
Moving from one point to the other along the segment $\lambda x_1^{(0)}  + (1-\lambda)x_2^{(0)}$  for $0\leq\lambda \leq 1$ we can evaluate the deep neural network $F$ at regular intervals.
More formally, define $\bm v = x_2^{(0)} - x_1^{(0)}$ and consider the points 
$x_1^{(0)} + \frac{t}{n} \bm v$ for $t \in [0,\ldots,n]$.
If two consecutive points are in the same linear cell we will have that 
\begin{equation} \label{eq:partial_d}
    \frac{F(\bm x_1^{(0)} + \frac{t+1}{n}\bm v) - F(\bm x_1^{(0)} + \frac{t}{n}\bm v)}{\frac{1}{n} ||\bm v||} = \frac{\partial F}{\partial \bm v}(\bm x_1^{(0)} + \frac{t}{n}\bm v).
\end{equation}
    
As the derivative of an affine function is constant, this vector will be constant inside each linear cell.
Moving along the segment, we might pass from one linear cell to a different one.
In this case we will notice a change in the derivative.
With a dichotomy, it is possible to identify the location of the critical point where this discontinuity is located.
Moving a little in a random direction from this point and using a similar technique, it is possible to identify other points on the same critical hyperplane until the whole hyperplane is determined. (i.e., we need $n_0$ independent points to determine the hyperplane of dimension $n_0 -1$ corresponding to the critical hyperplane)
Finally, the signature is collected by calculating an orthogonal vector $\bm w$ to this hyperplane and normalizing its first component to $1.$
In \cite{carlini2020} a slightly different method is proposed to recover the signature.


Notice that both $\bm w$ and $-\bm w$ are orthogonal vectors to the same plane but will share the same signature.
Crossing the hyperplane relative to a neuron corresponds to pass from an area where the neuron is active to an area where the same neuron is inactive or vice versa. The sign of $\bm w$ will determine which portion of the input space corresponds to the active area and which corresponds to the inactive area, determining the correct sign is then important to reconstruct the correct model.
In \cite{carlini2020}, the problem of determining the correct sign of each neuron resulted in exponential complexity in the number of neurons, as one could try to use all the possible combinations of signs until the correct one is found.
The attack was refined in \cite{canales23} were, thanks to the neuron wiggling technique, it was possible to predict the correct sign of each neuron with a certain accuracy.

A second challenge in this method, is that there is no guarantee that the signature collected is relative to a neuron in the first layer.
We will indeed measure a discontinuity in the first-order derivative every time a neuron in any layer switches between active and inactive.
In \cite{carlini2020}, it was observed that the hyperplanes relative to the nodes in the second and successive layers are bent by different activation patterns in the first layer.
This means that the signatures relative to the neurons in the first layer are always the same throughout the measurements, whereas the signatures relative to deeper nodes are ``distorted" in different ways.
Collecting enough signatures, it is possible to separate the signatures coming from the first layer (most frequent) from the one coming from deeper layers.
In this way, the authors of \cite{canales23} managed to recover the weights of a $4$-layer deep neural network. 
For deeper neural networks, distinguishing the signatures from the first layer becomes increasingly challenging.
Recently, \cite{liu2025} the limit was pushed to $8$ hidden layers, but in general deeper neural networks seem to be challenging in this regard.

\subsection{Our work}
As mentioned above, previous work focuses on recovering the rows of the weight matrices by identifying and using the borders of the linear cells. (i.e. portions of critical hyperplanes)

For a piecewise linear function $F$ and for a linear cell $C \in \R^{n_0}$ it is relatively easy to recover $F_{|C}.$
By definition $F_{|C}: C \rightarrow \R^{n_\ell}$ is an affine function which will be entirely determined by its value on $n_0 + 1$ independent points in $C.$
A naive idea would be to copy the function $F$ one cell at a time. 
Let $F$ be a $\Relu$ $\ell$-deep neural network. We denote by $n_k$ the number of neurons in the  $k$-th layer and by $N_h = n_1 + n_2+\ldots + n_{\ell-1}$ the number of neurons in all the hidden layers, then the number of distinct linear cells is upper bounded by $2^{N_h}$ \cite[Proposition 3]{montúfar2014}.
This bound is obtained by observing that each linear cell corresponds to a different activation pattern and there are at most $2^{N_h}$ possible distinct activation patterns.
In practice, some activation pattern might have no corresponding linear cell as there is no point in the input space that activates that precise pattern.
Even when the upper bound is not reached, the total number of linear cells is typically exponential in the number of neurons \cite{montúfar2014}.
Making the idea of coping $F$ one linear cell at a time extremely unpractical.

\iffalse
\color{blue}
\paragraph{FUTURE IDEA}\todo{Comment out in the final version. I left it as a reminder of what we could do.}: Suppose we know the architecture (i.e. how many layers and how many nodes per layer).
Although it is unpractical to determine the border and content of all linear cells, we can still determine the border and content of some of them.
Let say tht we determine the border and content of $n \leq N$ linear cells of $F$, where $N$ is the total number of linear cells in $F$ and let us call $\calC = \{C_1, \ldots, C_n \}$ the set containing the $n$ linear cells we determined.
Consider $\Tilde{F}$ a deep neural network with the same architecture of $F$ such that $\Tilde{F}_{C_i}=F_{|C_i}$ (i.e. $\Tilde{F}_{\calC}=F_{|\calC}$ ) for all $C_i \in \calC$, what is the minimum number of cells such that $\Tilde{F}=F$ throughout whole domain? 
Of course, if we choose $n=N$, as the union of all the cells corresponds already to the whole domain, we will have $\Tilde{F}=F$ in a trivial way. 
What is the smallest $\hat{n} \leq N$ such that for any given collection $\hat{\calC}$ of linear cells containing $\hat{n}$ linear cells such that $\Tilde{F}_{\hat{\calC}} = F_{\hat{\calC}} \Rightarrow \Tilde{F} = F$?

What is the smallest $n_{min}$ for which there exists a collection $\calC_{min}$ of linear cells such that $\Tilde{F}_{\calC_{min}} = F_{\calC_{min}} \Rightarrow \Tilde{F} = F$? (think of information set decoding as an analogy).

What could be the typical number $n_{avg}$ for which there exists a collection $\calC_{avg}$ of linear cells such that $\Tilde{F}_{\calC_{avg}} = F_{\calC_{avg}} \Rightarrow \Tilde{F} = F$?
(information set analogy: Given a random matrix $k \times n$ how many columns should we pick on average to get a matrix of rank $k$ with probability $P = 1-\epsilon$?)


If we relax a bit the condition on $\Tilde{F}$ and we look just to an approximation of $F$ (Don't know what should be the approriate distance to use but I would go for the $L_2$ distance over the compact set where our inputs can come from). Local copies of $F$ in some linear cells could be used to make an arbitrarily large amount of perfectly accurate training pairs $(\bm x, F(\bm x))$ from the same cell.
Generating those pairs on a sufficiently large number of distinct linear cells (maybe $n_{avg}$ or a bit more..) and use them to train a model as in \cite{tramer2016stealing} could give as a close approximation of the original model.
\color{black}
\fi

We will present a way to recover the columns of $\bm W^{(\ell)}$ comparing the local expression of the function $F$ in two adjacent linear cells.

Recall that a $\Relu$ $\ell$-deep neural network $F$ can be decomposed as
\begin{equation}
        \tag{\ref{eq:DNN}}
        F(\bm x) = A^{(\ell)} \circ \sigma^{(n_{\ell -1})} \circ \cdots \circ A^{(2)} \circ \sigma^{(n_1)} \circ A^{(1)}(\bm x),
        \end{equation}
where $\sigma = \Relu$ and each $A^{(k)}$ corresponds to the affine functions 
\begin{equation}\tag{\ref{eq:affine_function}}
        A^{(k)} = \bm W^{(k)} \bm x + \bm b^{(k)}.
    \end{equation}
We can define an intermediate function $H^{(i)}$ (head) as 
\begin{equation}\label{eq:F_int}
    H^{(i)}(\bm x) = \sigma^{(i)} \circ A^{(i)} \circ \cdots  \circ  \sigma^{(1)} \circ  A^{(1)}( \bm x).
\end{equation}
When we apply an intermediate function to a vector $\bm x^{(0)}  \in \R^{n_0},$ we obtain the output of the $i$-th layer,
$\bm x^{(i)} = F^{(i)}(\bm x^{(0)}).$
Extending this notation, the function $F$ can be denoted as $F^{(\ell)}$ and the output will be $F^{(\ell)}(\bm x^{(0)}) = \bm x^{(\ell)}$.
\color{blue}
Similarly we can denote by $T^{(i)}$ (tail) the function containing the last $i$ layers of the function $F$, that is 
\begin{equation}
    \label{eq:F_end}
    T^{(i)}(\bm x) = A^{(\ell)} \circ \sigma \circ \cdots \circ \sigma \circ A^{(\ell - i)} 
\end{equation}
It is clear that $F = T^{(\ell - i)} \circ H^{(i)}$, in particular $H^{(\ell)} = T^{(\ell)} = F.$
Using this notation, we will present the signature extraction in a slightly different way than in \cite{carlini2020}.

The analysis of the resulting function $F$ can be divided into two parts. 
One that is independent from the input, given by $\bm W^{(k)}$ and $b^{(k)}$, and one given by the activation functions $\sigma^{(k)}$ which will depend on the input.


Once we fix a particular input, this will determine a particular configuration of active-inactive neurons.
Each of these patterns can be represented by substituting the functions $\sigma^{(k)}$ with a diagonal matrices whose diagonal entries are $1$ if $\bm w_j^{(i)\perp} \bm x^{(i-1)} + b_j^{(i)} > 0$  (i.e. the corresponding neuron is active) and $0$ otherwise.
Each point in the input space $\bm x \in \R^{n_0}$ lies inside a linear cell or on the border between two.
As the borders are constituted by portions of hyperplanes having measure zero, a random point $\bm x$ will be inside a linear cell with probability $1.$ (In practice this probability will be only close to $1$ as we cannot have infinite precision).

For a given $\bm x_0$ we can denote the linear cell containing $\bm x_0$ as $[\bm x_0]$, for ease of notation we will denote simply by $ F_{| \bm x_0}$ the restriction of the function $F$ to $[\bm x_0].$
Locally (when restricted to  $[\bm x_0] \subseteq \R^{n_0}$) the function $F$ is a composition of affine functions and is therefore affine.
In particular we can write it as
\begin{equation*}
    F_{| \bm x_0} (\bm x) = \bm G_{|\bm x_0} \bm x + \bm b_{|\bm x_0}
\end{equation*}
The function $G_{| \bm x_0}(\bm x) = F_{|\bm x_0}(\bm x_0 + \bm x) - F_{|\bm x_0}(\bm x_0 ) $ is linear provided that $\bm x_0 + \bm x \in [\bm x_0]$.
From (\ref{eq:DNN}), we have that
\begin{equation}\label{eq:G_def}
    G_{|\bm x_0}(\bm x) = \bm W^{(\ell)} \sigma_{|\bm x_0}^{(\ell-1)} \cdots \sigma_{| \bm x_0}^{(1)} \bm W^{(1)} \bm x,
\end{equation}
as each linear cell corresponds to a particular activation pattern, with $\sigma_{|\bm x_0}^{(i)}$ we denote the $\Relu$ function at the $i$-th layer when the input is in $[\bm x_0],$ this corresponds to a diagonal matrix whose diagonal entries are $1$ for active neurons in the $i$-th layer and $0$ otherwise. 
\begin{lemma}\label{lm:G_const}
    Let $\bm x_0, \bm x_0' \in [\bm x_0]$
    In the intersection of their respective domains, the functions $G_{|\bm x_0}$ and $G_{|\bm x_0'}$ are the same function given in (\ref{eq:G_def}).
\end{lemma}
\begin{proof}
    For $\bm x_0'$ the function $G_{|\bm x_0'}$ is defined as
    $$
        G_{|\bm x_0'}(\bm x) = \bm W^{(\ell)} \sigma_{|\bm x_0'}^{(\ell-1)} \cdots \sigma_{| \bm x_0'}^{(1)} \bm W^{(0)} \bm x.
    $$
    Since $\bm x_0' \in [\bm x_0]$ the input $\bm x_0'$ will activate the neurons of the neural network in the same way as $\bm x_0,$ therefore $\sigma_{| \bm x_0'}^{(k)} = \sigma_{| \bm x_0}^{(k)}$ then $ G_{|\bm x_0'} =  G_{|\bm x_0}.$
\end{proof}


Similarly to (\ref{eq:F_int}) we can introduce the notation $G^{(i)}_{| \bm x_0} = \bm W^{(i)} \sigma_{|\bm x_0}^{(i)} \cdots \sigma_{| \bm x_0}^{(1)} \bm W^{(0)}.$
The functions $G_{| \bm x_0}(\bm x)$ and $\frac{\partial F}{\partial \bm v}(\bm x)$ in (\ref{eq:partial_d}) are deeply connected, for $\bm x_0 + \frac{t}{n} \bm v \in [\bm x_0]$, we have 
$$
\frac{\partial F}{\partial \bm v}\left (\bm x_0 + \frac{t}{n}  \bm v \right) = \frac{F(\bm x_0 + \frac{t+1}{n}\bm v) - F(\bm x_0 + \frac{t}{n}\bm v)}{\frac{1}{n} ||\bm v||} = \frac{ G_{|\bm x_0}\left (\frac{1}{n} \bm v \right )}{\frac{1}{n}||\bm v||} = \frac{G_{|\bm x_0}\left (\bm v \right )}{||\bm v||},
$$
where we used Lemma \ref{lm:G_const} for $G_{|\bm x_0 + \frac{t}{n}\bm v} = G_{|\bm x_0}$ in the second equality and the linearity of $G_{|\bm x_0}$ in the third.
In short, the above can be written as
\begin{equation}\label{eq:partial_FG}
    \frac{\partial F}{\partial \bm v}\left (\bm x_0 \right) = \frac{G_{|x_0}(\bm v)}{||\bm v||}.
\end{equation}

Consider $\bm x_0, \bm x_1$ belong to two adjacent linear cells, the two functions $G_{|\bm x_0},  G_{| \bm x_1}$ only differ by one entry in one of the $\Relu$ functions.

Suppose that $\sigma_{|\bm x_0}^{(\ell -1)} \neq \sigma_{|\bm x_1}^{(\ell -1)}$ then, since $\sigma_{|\bm x_0}^{(k)} = \sigma_{|\bm x_1}^{(k)}$ for all $k<\ell -1$, we have that $G_{|\bm x_0}^{(\ell -1)}( \bm v) = G_{|\bm x_1}^{(\ell -1)}( \bm v) = \bm y$ while $G_{|\bm x_0}^{(\ell)}( \bm v) \neq G_{|\bm x_1}^{(\ell)}( \bm v).$
In particular we have
$$
    G_{|\bm x_0}^{(\ell)}( \bm v) = \bm W^{(\ell)} \sigma_{|\bm x_0}^{(\ell -1)} \bm y \neq  \bm W^{(\ell)} \sigma_{|\bm x_1}^{(\ell -1)} \bm y = G_{|\bm x_1}^{(\ell)}( \bm v).
$$
Recall that the difference between $\sigma_{|\bm x_0}^{(\ell -1)}$ and $\sigma_{|\bm x_1}^{(\ell -1)}$ is just in one entry of the diagonal, without loss of generality we can consider the case where this entry is the first element of the diagonal.
Then
$$
    G_{|\bm x_0}^{(\ell)}( \bm v) - G_{|\bm x_1}^{(\ell)}( \bm v)  = \bm W^{(\ell)} \bm E_{1,1} \bm y = \bm W^{(\ell)}_{*,1} y_1,
$$
where we used the standard notation  $\bm E_{i,j}$ to denote the matrix that is zero everywhere except in its $(i,j)$-th entry where it is $1.$
The vector $\hat{\bm w}_{*,1}^{(\ell)}=\bm W^{(\ell)}_{*,1} y_1$ is proportional to the first column of $\bm W^{(\ell)}_{*,1}$ so we can get a \textbf{column-signature} of $\bm W^{(\ell)}_{*,1}$ from $\hat{\bm w}_{*,1}^{(\ell)}$.

When there is just one hidden layer, we are always in the case where the two cell differ by a neuron in the last (and only) layer.
Repeating the procedure we used to recover $\hat{\bm w}_{*,1}^{(\ell)}$ for different pairs of adjacent cells, we can collect several column signatures.
Assume that each neuron $\eta^{(\ell)}_1, \ldots, \eta^{(\ell)}_{n_{\ell}},$ has a non-null probability $p_1, \ldots, p_{n_{\ell}} > 0$ to switch and that $p = \min\{ p_1, \ldots, p_{n_{\ell}}\}$. 
The hardest column-signature to get will be the one corresponding to the neuron that is the least likely to switch.
We expect to observe this column-signature on average after $1/p$ attempts. (see geometric distribution) 
 
Unfortunately, when we consider more than one hidden layer, we can collect column-signature that do not correspond to the column of the matrix $\bm W^{(\ell)}.$
In general, there is no way to check if two different cells differ in the last layer or in an intermediate one.
With a similar argument to \cite{carlini2020} and \cite{canales23}, we could expect that signatures corresponding to the columns of the last matrix will have an higher frequency than signatures observed as a consequence of a switch in some intermediate state.
To see that, suppose
$
    G_{|\bm x_0}^{(k)}( \bm v) = G_{|\bm x_1}^{(k)}(\bm v) = \bm y
$
and that $k$ is the last layer for which this is true, then
$
    G_{|\bm x_0}^{(\ell)}( \bm v) \neq G_{|\bm x_1}^{(\ell)}(\bm v),
$
and in particular
\begin{align}\label{eq:bad_signature}
    G_{|\bm x_0}^{(\ell)}( \bm v) - G_{|\bm x_1}^{(\ell)}(\bm v)  & = \bm W^{(\ell)} \sigma_{|\bm x_0}^{(\ell-1)} \cdots \bm W^{(k+2)} \sigma_{|\bm x_0}^{(k+1)}  \bm W^{(k+1)} \bm E_{j,j} \bm y 
    \nonumber \\ & = \bm W^{(\ell)} \sigma_{|\bm x_0}^{(\ell-1)} \cdots \bm W^{(k+2)} \sigma_{|\bm x_0}^{(k+1)}  \bm W^{(k+1)}_{*,j} y_j
\end{align}
    

If there are $\bm x_0',\bm x_1'$ that also differ by the ReLU in the same layer $(k)$ at the same position $j$  the column vector $\bm W^{(k+1)}_{*,j} y_j'$ will be proportional (i.e. share the same signature) to $\bm W^{(k+1)}_{*,j} y_j$ in (\ref{eq:bad_signature}).  As the linear transformation $\bm W^{(\ell)} \sigma_{|\bm x_0'}^{(\ell-1)} \cdots \bm W^{(k+2)} \sigma_{|\bm x_0'}^{(k+1)}$ is in general different from the transformation $\bm W^{(\ell)} \sigma_{|\bm x_0}^{(\ell-1)} \cdots \bm W^{(k+2)} \sigma_{|\bm x_0}^{(k+1)}$ in (\ref{eq:bad_signature}) the two similar vectors will be twisted in different ways resulting in vectors that will probably not share the same signature.
This means, that if we do many samples, the vectors originated by a switch of a neuron in the last layer will have the tendency to repeat more often, enabling us to distinguish them and reconstructing the most external matrix $\bm W^{(\ell)}$.

Unfortunately, our experiments seem to support this analysis only when we consider a neural network with at most $2$ hidden layers.\todo{we need results to show. Also, we need better understanding what happens: after two layers, all abrublty breaks or is it gradual decrease in performance?}
What happens in real experiments with $\ell >2$ layers is that there are signatures originated in the last layer that we discard because they appear with a very low frequency (or do not appear at all) and signatures coming from internal layers that appear with a relatively high frequency.

\paragraph{Determination of sign}
Determining the correct sign for the column-signatures is considerably easier than for the row-signatures in the previous works \cite{carlini2020}, \cite{canales23}.
Suppose that we manage to recover and distinguish all the column-signatures of the matrix $\bm W^{(\ell)}$ and denote by $\hat{\bm W}^{(\ell)}$ the matrix whose columns are those signatures. 
To determine the correct sign of these columns, we can start by setting them  positive (i.e. having the first non-zero component positive).
Observe that each component of $\bm x^{(\ell -1)}$ is the output of a $\Relu,$ the solution $\bm y$ to
$$
    \hat{\bm W} \bm y + \bm b^{(\ell)} = \bm x^{(\ell)}
$$
must have all its components $\geq 0.$ 
If some components of $\bm y$ are negative we can multiply the corresponding column in $\hat{\bm W}$ by $-1$, in this way we will force each component of the solution to be positive and we determine the correct sign of each signature.


\paragraph{Bias recovery} 
Starting their attack from the first layer, Carlini et al. could determine the critical point $\hat{\bm x}$ for which $\bm w_i^{\intercal} \bm \hat{\bm x} + b_i = 0,$ from this equation it is easy to recover the value of the $i$-th component of the bias vector $\bm  b$ as $b_i = -\bm w_i^{\intercal} \bm \hat{\bm x}.$

In our case, once we collect all the column-signatures from $\bm W^{(\ell)},$ consider different inputs $\bm x_i^{(0)}$ indexed by $i \in I,$ we will have $\bm y_i = \bm x_i^{(\ell -1)}, \bm x_i^{(\ell)}$ satisfying the equation
\begin{equation}\label{eq:Wy+b=x}
    \bm W^{(\ell)} \bm y_i + \bm b^{(\ell)} = \bm x_i^{(\ell)}.
\end{equation}
In our model we do not know exactly $\bm W^{(\ell)}$ but we know the matrix $\hat{\bm W}^{(\ell)}$ whose columns $\hat{\bm w}_1, \ldots,\hat{\bm w}_m$ are the column signatures of the columns of $\bm W^{(\ell)}.$ 
The relation between the original weights $\bm W^{(\ell)}$ and the signature matrix is given by $\hat{\bm W}^{(\ell)} = \bm W^{(\ell)} \bm M$ where $\bm M = \bm P \bm D$ is the product between a permutation $\bm P$ and a diagonal matrix $\bm D.$
If there is a solution $\bm y_i$ for (\ref{eq:Wy+b=x}) then $\hat{\bm y}_i = \bm M^{-1} \bm y_i$ will be a solution of
\begin{equation}\label{eq:hat_Wy+b=x}
    \hat{\bm W}^{(\ell)} \hat{\bm y}_i + \bm b^{(\ell)} = \bm x_i^{(\ell)}.
\end{equation}
For each of these equations, the weight matrix $\hat{\bm W}^{(\ell)}$ and the outputs $\bm x_i^{(\ell)}$ are known, but both $\hat{\bm b}^{(\ell)}$ and $\hat{\bm y}_i$ are unknown.
From (\ref{eq:hat_Wy+b=x}) it follows that $\bm x_i^{(\ell)} \in \Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm b^{(\ell)}}$ for all $i,$ then $\bm b^{(\ell)} \in \cap_{i\in I} \Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm x_i^{(\ell)}}.$
When $\Rank(\hat{\bm W}^{(\ell)}) < n-1$ we the spaces $\Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm x_i^{(\ell)}} \subsetneq \R^{n_\ell}$ are strictly contained in $\R^{n_\ell}$ then, after sufficiently many intersections we can find a space $\Span{\R}{\bm b}$ of dimension $1$ containing $\bm b^{(\ell)}.$
Solving $\hat{\bm W}^{(\ell)} \bm y_i +  \lambda \bm b = \bm x_i$ in both $\bm y_i$ and $\lambda$ will give us the value of $\bm y_i$ and $\lambda,$ from which we will finally get the correct bias $\hat{\bm b}^{(\ell)} = \lambda \bm b.$
\color{black}

%\subsection{Where it fails}


\color{blue}
\section{Experiment and interpretation}
\todo{Section to be rewritten after experiments. Ignore it at the moment.}
\paragraph{Practical Issue}
In our experiment what stated above can be observed for $2-3$ layers at best.
What is happening in general and especially when we do have more hidden layer $>4,$ is that there are some columns belonging to $\bm W^{(\ell)}$ that do not appear very frequently or never.
At the contrary there are some column vectors that do appear very frequently even if they do not belong to the last layer.

An explanation could be that some neurons of the last layer flip very rarely in our experiment and that the same ``late" pattern $\bm W^{(\ell)} \sigma_{|\bm x_0'}^{(\ell-1)} \cdots \bm W^{(i+2)} \sigma_{|\bm x_0'}^{(i+1)}$ repeats in multiple experiments were the same at layer $i+1$ flips.

We ran our experiment only on a non-trained network that has a constant number of nodes per layer.
It might be that we can observe a better behavior for different kinds of nets and especially for a trained one.\todo{these are interesting experiments to show results}

Other ideas to improve would be to somehow identify areas in the input space where the last neurons are particularly stable or where they are more likely to flip.
In case this is possible we should concentrate our experiments on the areas where the last neurons flip more.
Could it be that the last layer is more active when we are close to a decision border? My intuition is that when the model is ``unsure" it will pass down the decision to the last layers while, if it is sure from the beginning, there will be not much to do for the nodes afterwards.\todo{I think this makes sense}
\\
\color{black}

The whole approach is very similar to what is happening in the case of Shamir and Carlini. 
We just flip output input, we observe what is happening inside the cells instead of determining their borders, we also can solve backward until we find a contracting layer while they can do forward until they find an expanding one.

\paragraph{Further development}
Consider how to combine the two techniques to handle both contracting and expanding.
Intuitively now we should be able to handle a network that is non expanding for some layer, after the first expansion we need it to be non contracting.  The shape of it will be a sort of $\bowtie.$ 

Another thing to consider is that the information contained in a linear cell is richer than what is in a border.
In particular a border can be "encoded" just by a vector describing the direction orthogonal to the border.
The linear part of a cell $G_{|\bm x_0}$ can have any dimension between $0$ and $d_{\min}$ where $d_{\min} = \min\{d_0, \ldots d_\ell\}$ denotes the layer having the least amount of neurons.
This leaves open the question if we can do better than just draw a line between two adjacent cells or if we could consider the whole expression of the function inside each cell we investigate and combine all these information in a meaningful way (see the paragraph ``FUTURE IDEA" a few pages ago).

==> SecondOrderNew.tex <==
\section{Two-Side Signature Recovery}
\label{sec:twoside}

An important property of DNNs having $\Relu$ or any other piecewise linear function as activation function is that they realize a function which is also piecewise-linear.
We will see how this property allows us to extract the neuron signatures. 

\begin{definition}[Piecewise linear function]
A function $F: \R^n \rightarrow \R^m$ is said to be \textbf{piecewise linear} if there exists a finite collection $\calC =\{C_1, \ldots, C_t \},$ where $C_i$ are the solution to a system of linear inequalities such that $\bigcup_{i=1}^t C_i = \R^n $ and
$$
    F_{|C_i}(\bm x) = \bm W_i \bm x + \bm b_i,
$$ 
where $F_{|C_i}$ denotes the restriction of $F$ to the set $C_i$ and $\bm W_i \in \R^{m \times n}, \bm b_i \in \R^{m}.$
In other words, the restriction of $F$ to the sets $C_i$ is an affine function.
The sets $C_i$ are also known as \textbf{linear cells}.
\end{definition}
An example of a piecewise linear function is given by $\Relu$.
\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=0.9]

% outer box just to frame the picture
\draw[thin, gray!40] (-4,-3) rectangle (4,3);

% hyperplanes
\draw[thick] (-4,-1.4) -- (4,1.5);
\draw[thick] (-1.5,-3) -- (-1.5,3);
\draw[thick] (-4,2.4) -- (4,-2);
%\draw[thick] (1.8,-3) -- (1.8,3);

% labels in some cells
\node at (-2.3,2.3) {$F_{\mid C_1}$};
\node at (1, 1.8) {$F_{\mid C_2}$};
%\node at (2.8,2.3) {$F_{\mid C_3}$};

\node at (-2.8,0.4) {$F_{\mid C_3}$};
\node at (-1.0,0.15) {$F_{\mid C_4}$};
\node at (2.7,0) {$F_{\mid C_5}$};

\node at (-2.8,-2) {$F_{\mid C_6}$};
\node at (1.1,-1.8) {$F_{\mid C_7}$};
%\node at (2.7,-2.0) {$F_{\mid C_9}$};

\end{tikzpicture}
\caption{A subdivision of $\mathbb{R}^2$ into linear cells. On each cell $C_i$, the restriction $F_{\mid C_i}$ of $F$ is affine.}
\label{fig:linear-cells}
\end{figure}

The composition of affine functions and piecewise linear functions (in this case, the $\Relu$ function) results in piecewise linear functions whose linear cells are delimited by portions of hyperplanes.
As anticipated, the function $F$ in Definition \ref{def:DNN} corresponds exactly to this case and is therefore a piecewise linear function.

Recall from Definition \ref{def:DNN} that the function implemented by a neural network can be described as
\begin{equation}
\tag{\ref{eq:DNN}}
F(\bm x) = A^{(\ell)} \circ \bm \sigma \circ \cdots \circ A^{(2)} \circ \bm \sigma \circ A^{(1)}(\bm x),
\end{equation}

where $A^{(k)}(\bm x) = \bm W^{(k)} \bm x  + \bm b^{(k)}$ for some weight matrix $\bm W^{(k)} \in \R^{n_n \times n_{k-1}}$ and bias vector $\bm b^{(k)} \in \R^{n_k}$ that do not depend on the input.
On the contrary, the activation functions $\bm \sigma$ will activate in a different manner according to the input $\bm x.$

Once we fix a particular input, this will determine a particular configuration of active-inactive neurons.
Each of these patterns can be represented by substituting the function $ \bm \sigma$ at layer $k$ with a diagonal matrix whose diagonal entries are $1$ if $\bm w_{i,*}^{(k)\intercal} \bm x^{(k-1)} + b_i^{(k)} > 0$  (i.e., the corresponding neuron is active) and $0$ otherwise.
Each point in the input space $\bm x \in \R^{n_0}$ lies within a linear cell or on the border between two.
As the borders are constituted by portions of hyperplanes having measure zero, a random point $\bm x$ will be inside a linear cell with probability $1$.\footnote{In practice, this probability will be only close to $1$ as we cannot have infinite precision.}

For a given $\bm x_0$, we can denote the linear cell containing $\bm x_0$ as $ C_0$, we will denote by $ F_{| C_0}$ the restriction of the function $F$ to the cell $C_0.$
Locally (when restricted to  $ C_0 \subseteq \R^{n_0}$), the function $F$ is a composition of affine functions and is therefore affine.
If we denote by $\bm \sigma_{|C_0}^{(k)}$ the diagonal matrix representing the activation state of the $k$-th layer over the linear cell $C_0$, we can write 
\begin{equation}
\label{eq:F=G+b}
    F_{| C_0} (\bm x) = \bm G_{|C_0} \bm x + \bm b_{|C_0}
\end{equation}
where $\bm G_{|C_0} = \bm W^{(\ell)} \bm \sigma_{|C_0}^{(\ell-1)} \cdots \bm \sigma_{|C_0}^{(1)} \bm W^{(1)} \in \R^{n_\ell \times n_0}$ 
and 
$\bm b_{|C_0} = \sum_{i=1}^\ell \bm C^{(i)}_{|C_0}  \bm b^{(i)}$ where
$\bm C^{(i)}_{|C_0} = \bm W^{(\ell)}\bm \sigma^{(\ell-1)}_{|C_0} \cdots \bm W^{(i+1)} \bm \sigma_{|C_0}^{(i)}$ 
for $i< \ell$ and $\bm C_{|C_0}^{(\ell)}= I_{n_\ell}$ is equal to the identity.
The image of $F_{|C_0}$ will have dimension equal to the rank of the matrix $\bm G_{|C_0}$. Informally, we will refer to this as the dimension of $F_{|C_0}.$
To determine an affine function of dimension $d$, it is sufficient to know its evaluation over $d+1$ independent points.
Then, it is always possible to determine the function $F_{|C_0}$ and the matrix $\bm G_{|C_0}.$
Another interpretation of the matrix $\bm G_{|C_0}$ is that it is the Jacobian of the function $F_{|C_0}$ that is
\begin{equation}
\label{eq:G_Jacobian}
    \bm G_{|C_0} = 
    \begin{pmatrix}
\frac{\partial F_{1|C_0,}}{\partial x_1} & \frac{\partial F_{1|C_0}}{\partial x_2} & \cdots & \frac{\partial F_{1|C_0}}{\partial x_{n_0}} \\
\frac{\partial F_{2|C_0,}}{\partial x_1} & \frac{\partial F_{2|C_0}}{\partial x_2} & \cdots & \frac{\partial F_{2|C_0}}{\partial x_{n_0}} \\
\vdots & \vdots & \ddots & \vdots \\
\frac{\partial F_{n_{\ell}|C_0,}}{\partial x_1} & \frac{\partial F_{n_{\ell}|C_0}}{\partial x_2} & \cdots & \frac{\partial F_{n_{\ell}|C_0}}{\partial x_{n_0}} 
\end{pmatrix},
\end{equation}
where $\frac{\partial F_{i|C_0,}}{\partial x_j}$ is the partial derivative in direction $x_j$ of the $i$-th component of the function $F_{|C_0}.$

This simple fact becomes crucial when we compare the function in two adjacent linear cells, that is, two linear cells divided by a portion of a critical hyperplane.
Let $[\bm x_0]$ and $[\bm x_1]$ be two adjacent linear cells that differ only in the activation of the $j$-th neuron of the $i$-th layer.
The diagonal matrices satisfy $\bm \sigma_{|C_0}^{(k)} = \bm \sigma_{|C_1}^{(k)}$ for all $k \neq i$ while $\bm \sigma_{|C_0}^{(i)} - \bm \sigma_{|C_1}^{(i)} = \pm \bm E_{j,j}$ where $\bm E_{j,j} \in \R^{n_i \times n_i}$ is the matrix that is $0$ in each entry except in the position $(j,j)$ where it is $1.$
The decomposition of 
$$
    \bm G_{|C_0} = \bm W^{(\ell)} \bm \sigma_{|C_0}^{(\ell-1)} \cdots \bm \sigma_{|C_0}^{(1)} \bm W^{(1)}
$$
can be conveniently grouped into a tail 
$$
    \bm T_{|C_0}^{(\ell - i)} = \bm W^{(\ell)} \bm \sigma_{|C_0}^{(\ell-1)} \cdots \bm \sigma_{| \bm x_0}^{(i+1)} \bm W^{(i+1)},
$$
the activation map relative to the $i$-th layer $\sigma_{|C_0}^{(i)}$ and a head 
$$
    \bm H^{(i)}_{|C_0} = \bm W^{(i-1)} \bm \sigma_{|C_0}^{(i-1)} \cdots \bm \sigma_{|C_0}^{(1)} \bm W^{(1)}
$$
giving the decomposition
\begin{equation}
\label{eq:G=TsH}
    \bm G_{|C_0} = \bm T_{|C_0}^{(\ell - i)} \bm \sigma_{|C_0}^{(i)} \bm H^{(i)}_{|C_0}.
\end{equation}
    
As $\bm G_{|C_0}$ and $\bm G_{|C_1}$ share the same head $\bm H_{|C_0}^{(i)}$ and tail $\bm T_{|C_0}^{(\ell - i)}$  and $\bm \sigma_{|C_0}^{(i)} - \bm \sigma^{(i)}_{|C_1} = \bm E_ {j,j}$ their difference is the matrix of rank $1$ given by
\begin{equation}
\label{eq:Signature_as_rank1}
    \bm G_{|C_0} - \bm G_{| C_1} = \bm T_{|C_0}^{(\ell -i)} \bm E_{j,j} \bm H_{|C_0}^{(i)} = \bm t_{*,j} \bm h_{j,*}^{\intercal},
\end{equation}
where $\bm t_{*,j}$ is the $j$-th column of $\bm T_{\bm x_0}^{(\ell -i)}$ and $\bm h_{j,*}^\intercal$ is the $j$-th row of $\bm H_{|C_0}^{(i)}$.

Each row of the matrix $\bm G_{|C_0} - \bm G_{| C_1}$ is a scalar multiple of the row vector $\bm h_{j,*}^\intercal$. The same is true for its columns, which are all scalar multiples of the column vector $\bm t_{*,j}$. 
In terms of Definition \ref{def:signature}, every row of $\bm G_{|C_0} - \bm G_{| C_1}$ has the same row-signature and every column has the same column-signature. 

\todo{maybe some subsection?}
There are two special cases in which we can exploit this decomposition to recover the row-signatures or the column-signatures of the matrices $\bm W^{(i)}$.

The first case is when the activation patterns for $C_0$ and $C_1$ differ for the $j$-th neuron in the first layer, then, since $\bm H^{(1)} = \bm W^{(1)},$  each row of the matrix $\bm G_{|C_0} - \bm G_{| C_1}$ is a scalar multiple of the $j$-th row of $\bm W^{(1)}$.
This is exactly the same case exploited in \cite{carlini2020} and the following works.
The connection is even more evident if we recall that $\bm G_{|C_0}$ is the Jacobian of the local affine function $F_{|C_0}(\bm x).$ 

The second and new case is if the activation patterns differ in the $j$-th neuron of the last layer, since $\bm T^{(1)} = \bm W^{(\ell)},$ the columns of $\bm G_{|C_0} - \bm G_{\mid C_1}$ will be a scalar multiple of the $j$-th column of $\bm W^{(\ell)}$.

As already stated, the first case was exploited to collect all the signatures of the first layer and from there attack the second layer, and so on.
Then, a natural question arises: Can we follow a similar approach, collecting the column signature of the last layer, and proceed backwards towards the first?
If successful, then the two approaches could be easily combined, reconstructing the function from both ends.

\subsection{Locating Linear Cell Borders}

\todo{I find the description in this section (and the next ones) very "wordy". Can we express this with mathematical 
equations?}

To find signatures, it is essential to find adjacent linear cells.
A method to do so is to select two inputs $\bm x_0^{(0)}, \bm x_1^{(0)}$ and move along a segment that connects them, evaluating the function $F$ at regular intervals.
The segment can be parametrized by $0\leq\lambda \leq 1$
as 
$\lambda \bm x_0^{(0)}  + (1-\lambda) \bm  x_1^{(0)}.$ 
More formally, define $\bm v =\bm  x_1^{(0)} - \bm x_0^{(0)}$ and consider the points 
$\bm x_0^{(0)} + \frac{t}{n} \bm v$ for $t \in [0,\ldots,n]$.
If two consecutive points are in the same linear cell, we will have that 
\begin{equation} \label{eq:partial_d}
    \frac{F(\bm C_0^{(0)} + \frac{t+1}{n}\bm v) - F(\bm C_0^{(0)} + \frac{t}{n}\bm v)}{\frac{1}{n} ||\bm v||} = \frac{\partial F}{\partial \bm v}\left (\bm C_0^{(0)} + \frac{t}{n}\bm v \right ).
\end{equation}
    
As the derivative of an affine function is constant, this vector will be constant inside each linear cell.
In particular, the vector will correspond to $\bm G_{|\bm c_i} \frac{\bm v}{||\bm v ||}$ where $[\bm c_i]$ denotes the linear cell that contains both $\bm C_0^{(0)} + \frac{t}{n}\bm v$ and $\bm C_0^{(0)} + \frac{t+1}{n}\bm v$. 
Moving along the segment, we might pass from one linear cell to another.
In this case, we will notice a change in the derivative.
\color{blue}
This method slightly differs from \cite{carlini2020} and subsequent works, which restrict the function $F$ to a single component.
In their case, the derivative is then just a scalar corresponding to one component of the vector we are monitoring.
They spot a change in the linear cell  whenever this scalar changes.
In principle, for $[\bm C_0],[\bm C_1]$ different linear cells, the vectors $\frac{\partial F}{\partial \bm v}\left (\bm C_0^{(0)} \right )$ and $\frac{\partial F}{\partial \bm v}\left (\bm C_1^{(0)} \right )$ could be different but being equal in the component to which we restricted.
In this case, the method in \cite{carlini2020} would fail to distinguish $[C_0],[C_1]$ as two distinct linear cells.
As this event has measure zero, this was not considered an issue.
\color{black}
With a dichotomy, it is possible to identify the location of the critical point where this discontinuity is located.
\color{blue}

\paragraph{Row-signature extraction}
In \cite{carlini2020} the row-signature is found by comparing the  difference in the derivative on the two sides of the critical plane for sufficiently many independent directions $\bm v$ and solving a linear system.
An equivalent technique proposed in \cite{chen2024hard} is to move a little in a random direction from the individuated critical point and find another one.
Once sufficiently many independent critical points are found (i.e.,  $n_0$ independent points are enough to determine the hyperplane of dimension $n_0 -1$ corresponding to the critical hyperplane), it is possible to find the whole critical hyperplane, and the row signature will correspond to the vector orthogonal to it.

Both of these methods suffer from the same problem of not being able to recover a signature if it is not possible to find enough linearly independent equations or independent points on the critical hyperplane.
This is equivalent to ask that the image of function $F$, evaluated only up to the layer $k$, has dimension $n_k$.
Informally we refer to the dimension of the image of $F$ as the rank of $F.$
For any layer following an expansion ,i.e. any layer $L_k$ such that $|L_{k-1}| < |L_k|$, the rank of $F$ evaluated up to the layer $k$ is at most $n_{k-1} < n_k$ so in theory it is impossible to recover the signature.
Due to the presence of $\Relu$, the function $F^{(k)}_{|\bm C_0}$ can have a rank smaller than $n_k$ even if all the previous layers were larger than $n_k$.
This phenomenon is known as rank loss and is a limiting factor for the signature recovery in \cite{carlini2020}.
In \cite{liu2025}, this problem was resolved by combining linear equations coming from distinct portions of hyperplanes relative to the same neuron. 
The key observation is that this would give a one-dimensional space if two or more of the equations are relative to the same neuron, while it would give no solution if the equations were relative to distinct neurons.


\color{black}
\todo{we need to be clear what is done in [6] and what we do - at least at the level of a more general formula}

\color{blue}
\subsubsection{Comparison to our extraction}
In the previous subsection we explained how, using the partial derivative $\frac{\partial F}{\partial \bm v}$, it is possible to find subsequent linear cells.
Let $[\bm C_0], [\bm C_1]$ be two subsequent linear cells, from Eq.~\eqref{eq:Signature_as_rank1}
we can get a rank $1$ matrix $\bm \Delta(C_0, C_1) = \bm G_{|\bm C_0} - \bm G_{|\bm C_1}.$ \todo{introduce some nicer notation for $S$ somewhere, maybe right after Eq. ~\eqref{eq:Signature_as_rank1}, propose $\Delta^{\bm C_1} \bm G_{|C_0}$ or $\bm S_{\bm C_0,\bm C_1}$}
We already discussed how, if the activation pattern of $\bm C_0$ differs from the activation pattern of $[\bm C_1$ in the first layer, the rows of $\bm \Delta(C_0, C_1)$ have the same row signature of a neuron of the first layer while, if the difference is in the last layer, the columns of $\bm \Delta(C_0, C_1)$ share the same column-signature of one column of $\bm W^{(\ell)}$.
Central layers will be recovered once we determine the most externals.

Our method presents similar limitations in terms of rank as the one in \cite{carlini2020} we described in the previous paragraph.\todo{unclear what is done by us and what not}
In particular, if the signature we are recovering is from the first or last layer, we directly obtain a row or column signature.
For deeper (central) layers, we assume to know the head $\bm H^{(i-1)}$, or the tail $\bm T^{(\ell-i)}$.
The row signature we recover at an internal layer is passed through the head, and the column signature through the tail.
This means we can obtain the original signature only if we can invert the head or the tail, respectively.
When these matrices are not invertible (under-determined), the solution will not be unique.
In this case, we can still use a similar approach to that in \cite{liu2025}.
That is, we can match two signatures from the same level, which, in principle, will have a different head or tail.
If the two signatures refer to different neurons or columns, there will be no solution, while if they refer to the same neuron or column, there will be a unique solution.
Columns are theoretically easier to determine in the case of expanding networks as the tail will be more overdetermined, on the contrary, contracting networks favor the head to be overdetermined making comparatively easier to recover row-signatures.
A network that only contracts should be easier to recover using the row signature while a network that only expand (not really useful in practice) should be easier to attack from the tail using column signatures.
A network that starts with some contraction and ends with some expanding layers (such as autoencoder) should be easier to attack on both side until we meet in the narrowest layer.

\paragraph{Enhance precision}
Due to numerical errors the recovery of the signatures will always have some error.
These errors will accumulate when we explore deeper layers, this affect both the fidelity of the reconstructed model and the capacity to reliably extract deep layers.

In previous works, signatures were collected as single row-signatures and grouped by similarity fixing a threshold distance.
In our case, the matrix $\bm \Delta(C_i, C_j)$ will contain rows (or columns) referring all to the same signature.
A way to increase the precision is naturally given by (Singular Value Decomposition) SVD.
This technique should improve the precision of the signatures extracted.

If the entries correspond to non-adjacent cells, the matrix is no longer approximately rank-$1$; this is reflected in the presence of multiple significant singular values. 

\color{black}
\todo{I thought we would emphasize more on expanding layers?}

\subsection{Sign determination and layer attribution}
Collecting all the signatures of one layer is not sufficient if we cannot determine their signs as well.
If we think of of a row-signature as to the direction orthogonal to an hyperplane, we have that both $\bm w$ and $-\bm w$ are orthogonal vectors to the same hyperplane but share the same signature.
Crossing the hyperplane relative to a neuron corresponds to moving from an area where the neuron is active to an area where the same neuron is inactive or vice versa. The sign of $\bm w$ will determine which portion of the input space corresponds to the active area and which corresponds to the inactive area; determining the correct sign is then important to reconstruct the correct model.
In \cite{carlini2020}, the problem of determining the correct sign of each neuron results in exponential complexity in the number of neurons, since one could try to use all the possible combinations of signs until the correct one is found.
The attack was refined in \cite{canales23}, where, thanks to the neuron wiggling technique, it was possible to predict the correct sign of each neuron with a certain accuracy.


A second challenge when collecting signatures is that there is no guarantee that the signatures collected are relative to the layer we are attacking.
We will indeed measure a discontinuity in the first-order derivative every time a neuron in any layer switches between active and inactive.
In \cite{carlini2020}, it was observed that the hyperplanes relative to the nodes in the second and successive layers are bent by different activation patterns in the first layer.
This means that the signatures relative to the neurons in the first layer are always the same throughout the measurements, whereas the signatures relative to deeper nodes are ``distorted" in different ways.
Collecting enough signatures, it is possible to separate the signatures coming from the first layer (most frequent) from those coming from deeper layers.
In this way, \cite{canales23} managed to recover the weights of a $4$-layer deep neural network. 
For deeper neural networks, distinguishing the signatures from the first layer becomes increasingly challenging.
Recently, in \cite{liu2025}, the limit was pushed to $8$ hidden layers, but in general, deeper neural networks seem to be challenging in this regard.

\subsection{Sign and layer determination for two-side signatures}
\color{red}
TODO:
I think the first part of this section regarding copying the function piece by piece is interesting but not in the right position.
Probably the paper flows better if we explain how we address (actually fail to address in practice) the problem of signs and layer determination in the case of column-signatures.
Is there a place where we can still present this discussion? Maybe right after the piecewise linear definition and discussion at the beginning of the two side signature recovery section.
I remember the idea of exploiting this fact to create virtual extra evaluation points and train a network on them.
\color{black}
As mentioned above, previous work focuses on recovering the rows of the weight matrices by identifying and using the boundaries between two linear cells. (i.e., portions of critical hyperplanes)

For a piecewise linear function $F$ and for a linear cell $C \in \R^{n_0}$ it is relatively easy to recover $F_{|C}.$
By definition $F_{|C}: C \rightarrow \R^{n_\ell}$ is an affine function which will be entirely determined by its value on $n_0 + 1$ independent points in $C.$
A naive idea would be to copy the function $F$ one cell at a time. 
Recovering the affine expression of $F_{|C}$ presents similar challenges in terms of finding sufficiently many affine independent points to evaluate, as in the case of reconstructing the critical hyperplanes.

Let $F$ be a $\Relu$ $\ell$-deep neural network. We denote by $n_k$ the number of neurons in the  $k$-th layer and by $N_h = n_1 + n_2+\ldots + n_{\ell-1}$ the number of neurons in all the hidden layers. Then, the number of distinct linear cells is upper bounded by $2^{N_h}$ \cite[Proposition 3]{montúfar2014}.
This bound is obtained by observing that each linear cell corresponds to a different activation pattern and there are at most $2^{N_h}$ possible distinct activation patterns.
In practice, some activation patterns might have no corresponding linear cell, as there is no point in the input space that activates that precise pattern.
Even when the upper bound is not reached, the total number of linear cells is typically exponential in the number of neurons \cite{montúfar2014}.
This makes the idea of copying $F$ one linear cell at a time extremely impractical.

As we have shown in the previous section, recovering $F$ in adjacent cells can give us some information about the column signatures of $\bm W^{(\ell)}$ or row signatures of $\bm W^{(1)}$ in the case the two cell differ by a neuron in the last or the first hidden layer, respectively.

When there is just one hidden layer, we are always in the case where two adjacent cells differ by a neuron in the last (and only) layer.
This means that from different pairs of adjacent cells, we can collect several column signatures referring to the same layer.
Assume that each neuron $\eta^{(\ell)}_1, \ldots, \eta^{(\ell)}_{n_{\ell}},$ has a non-null probability $p_1, \ldots, p_{n_{\ell}} > 0$ to switch and that $p = \min\{ p_1, \ldots, p_{n_{\ell}}\}$. 
The hardest column signature to get will be the one corresponding to the neuron that is the least likely to switch.
We expect to observe this column-signature on average after $1/p$ attempts.
\todo{let us make a lemma? Ermes: I think the same is already informally discussed in \cite{carlini2020} or subsequent work as coupon collector problem, folklore?}
\color{red}
I think that we should avoid the verb "to expect", because it may cause confusion. Do we mean the mathematical operation "to compute the expected value of a random variable" or do we mean that we
are making an assumption that seems reasonable to us?
\color{black}
 
Unfortunately, when we consider more than one hidden layer, we can collect column-signatures that do not correspond to the column of the matrix $\bm W^{(\ell)}.$
In general, there is no way to check if two different cells differ in the last layer or in an intermediate one.
With a similar argument to \cite{carlini2020} and \cite{canales23}, we expect that signatures corresponding to the columns of the last matrix will have a higher frequency than signatures observed as a consequence of a switch in some intermediate state.
To justify this assumption, recall Eq.~\eqref{eq:Signature_as_rank1}.
For two linear cells $[\bm x_0], [\bm x_1]$ that differ in only in the activation of the neuron $\eta_{j}^{(i)}$ we have
$$
     \bm G_{|C_0} - \bm G_{| \bm x_1} = \bm T_{|C_0}^{(\ell -i)} \bm E_{j,j} \bm H_{|C_0}^{(i)} = \bm t_{*,j} \bm h_{j,*}^{\intercal}.
$$
Suppose there exist other two cells $[\bm x_2], [\bm x_3]$ that differ in the activation of the same neuron $\eta_j^{(i)}$.
If $i=\ell$, then we are on the last layer and we have $\bm T_{|C_0} = \bm T_{|c_2} = \bm W^{(\ell)}$, which means the matrices $\bm G_{|C_0} - \bm G_{| \bm x_1}$ and $\bm G_{|c_2} - \bm G_{| \bm x_3}$ will all share the same column $\bm w^{(\ell)}_{*,j}$ up to some scalar.
That is, we would observe the same signature twice.
In all the other cases, as there is no reason why the activation patterns relative to the layer $i+1$ to $\ell$ are the same for two different cells, we expect $\bm T_{|C_0}^{(\ell-i)} \neq \bm T_{|c_2}^{(\ell-i)}$.
Thus, while we find two independent transitions of the same neuron, we will observe two different column signatures.
The identical consideration is true for the row signatures once we observe that the only case in which we are sure $\bm H_{|C_0}^{(i)} = \bm H_{|c_2}^{(i)}$ is for $i=1$ where $\bm H_{|C_0}^{(1)} = \bm H_{|c_2}^{(1)} = \bm W^{(1)}.$
\color{blue}
A challenge for the whole process is that there is no guarantee that the frequency argument will let us attribute the signature to the correct layer.
In \cite{carlini2020}, it was observed that the hyperplanes relative to the nodes in the second and successive layers are bent by different activation patterns in the first layer.
This means that the signatures relative to the neurons in the first layer are always the same throughout the measurements, whereas the signatures relative to deeper nodes are ``distorted" in different ways.
This is clear from our model when we noticed that different linear cells have, in general, different heads.


Unfortunately, column signatures seem even more challenging in this regard.
From our experiments, the simple frequency approach let us distinguish signatures from the last layer from other signatures only with $1$ (trivial) or $2$ hidden layers.
As soon as we add more layers we observe many false positives (signatures with a high frequency that do not belong to the last layer) and many signatures from the last layer that, while present in the set of all the signatures we recover do not appear with a high enough frequency to distinguish them from the bulk of all the other signatures coming from inner layers.
\todo{we need results to show. Also, we need better understanding what happens: after two layers, all abrublty breaks or is it gradual decrease in performance?}

\todo{we need something more here, it does not make sense to develop a method/section and finish it in two lines...}

\color{black}


\paragraph{Determination of Sign}
Determining the correct sign for the column-signatures is considerably easier than for the row-signatures in the previous works \cite{carlini2020}, \cite{canales23}.
Suppose that we manage to recover and distinguish all the column-signatures of the matrix $\bm W^{(\ell)}$ and denote by $\hat{\bm W}^{(\ell)}$ the matrix whose columns are those signatures. 
To determine the correct sign of these columns, we can start by setting them positive (i.e., having the first non-zero component positive).
Observe that each component of $\bm x^{(\ell -1)}$ is the output of a $\Relu,$ then the solution $\bm y$ to
$$
    \hat{\bm W} \bm y + \bm b^{(\ell)} = \bm x^{(\ell)}
$$
must have all its components $\geq 0.$ 
If some components of $\bm y$ are negative, we can multiply the corresponding column in $\hat{\bm W}$ by $-1$; in this way, we will force each component of the solution to be positive, and we determine the correct sign of each signature.


\paragraph{Bias recovery} 
Starting their attack from the first layer, Carlini et al. \cite{carlini2020} could determine the critical point $\hat{\bm x}$ for which $\bm w_i^{\intercal} \bm \hat{\bm x} + b_i = 0,$. From this equation, it is easy to recover the value of the $i$-th component of the bias vector $\bm  b$ as $b_i = -\bm w_i^{\intercal} \bm \hat{\bm x}.$

In our case, once we collect all the column-signatures from $\bm W^{(\ell)},$ and consider different inputs $\bm x_i^{(0)}$ indexed by $i \in I,$ we will have $\bm y_i = \bm x_i^{(\ell -1)}, \bm x_i^{(\ell)}$ satisfying the equation
\begin{equation}\label{eq:Wy+b=x}
    \bm W^{(\ell)} \bm y_i + \bm b^{(\ell)} = \bm x_i^{(\ell)}.
\end{equation}
We do not know exactly $\bm W^{(\ell)}$ but we know the matrix $\hat{\bm W}^{(\ell)}$ whose columns $\hat{\bm w}_1, \ldots,\hat{\bm w}_m$ are the column signatures of the columns of $\bm W^{(\ell)}.$ 
The relation between the original weights $\bm W^{(\ell)}$ and the signature matrix is given by $\hat{\bm W}^{(\ell)} = \bm W^{(\ell)} \bm M$ where $\bm M = \bm P \bm D$ is the product between a permutation $\bm P$ and a diagonal matrix $\bm D.$
If there is a solution $\bm y_i$ for Eq.~\eqref{eq:Wy+b=x}, then $\hat{\bm y}_i = \bm M^{-1} \bm y_i$ will be a solution of
\begin{equation}\label{eq:hat_Wy+b=x}
    \hat{\bm W}^{(\ell)} \hat{\bm y}_i + \bm b^{(\ell)} = \bm x_i^{(\ell)}.
\end{equation}
For each of these equations, the weight matrix $\hat{\bm W}^{(\ell)}$ and the outputs $\bm x_i^{(\ell)}$ are known, but both $\hat{\bm b}^{(\ell)}$ and $\hat{\bm y}_i$ are unknown.
From Eq.~\eqref{eq:hat_Wy+b=x}, it follows that $\bm x_i^{(\ell)} \in \Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm b^{(\ell)}}$ for all $i,$ then $\bm b^{(\ell)} \in \cap_{i\in I} \Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm x_i^{(\ell)}}.$
When $\Rank(\hat{\bm W}^{(\ell)}) < n-1$ the spaces $\Span{\R}{\hat{\bm w}_1, \ldots, \hat{\bm w}_m, \bm x_i^{(\ell)}} \subsetneq \R^{n_\ell}$ are strictly contained in $\R^{n_\ell}$ then, after sufficiently many intersections we can find a space $\Span{\R}{\bm b}$ of dimension $1$ containing $\bm b^{(\ell)}.$
Solving $\hat{\bm W}^{(\ell)} \bm y_i +  \lambda \bm b = \bm x_i$ in both $\bm y_i$ and $\lambda$ will give us the value of $\bm y_i$ and $\lambda,$ from which we will finally get the correct bias $\hat{\bm b}^{(\ell)} = \lambda \bm b.$
\color{black}

%\subsection{Where it fails}







==> discussion.tex <==
\section{Discussion and Possible Defenses}

\subsection{Limitations when Extracting from the Last Layers}

\subsection{Adding Expanding Layers as a Defense}

\subsubsection{First Layers}

\subsubsection{Last Layers}


Possible directions:\\
We need to start with the simplest question: do we start from the beginning or end of NN? And can we combine our approach with Carlini/Shamir approach?\\
Next, the question is what happens in different architecture types of neural network:\\
1. a neural network that always remains constant or decreasing.\\
2. a neural network that always remains constant or decreasing except for one layer at the beginning that expands.\\
3. a neural network that always remains constant or decreasing except for one layer at the end that expands.\\
4. a neural network that always expands (like decoder in AE).\\

Regarding the increase in layer size, can we determine some bound that we can cover?


\todo{there were some more directions that we discussed during the meeting but I forgot. Gorka had opinion about something I said and I agreed, but I do not remember what was it...}


